Programming over Thinking: Efficient and Robust Multi-Constraint Planning

Multi-constraint planning involves identifying, evaluating, and refining candidate plans while satisfying multiple, potentially conflicting constraints. Existing large language model (LLM) approaches face fundamental limitations in this domain. Pure reasoning paradigms, which rely on long natural language chains, are prone to inconsistency, error accumulation, and prohibitive cost as constraints compound. Conversely, LLMs combined with coding- or solver-based strategies lack flexibility: they often generate problem-specific code from scratch or depend on fixed solvers, failing to capture generalizable logic across diverse problems. To address these challenges, we introduce the Scalable COde Planning Engine (SCOPE), a framework that disentangles query-specific reasoning from generic code execution. By separating reasoning from execution, SCOPE produces solver functions that are consistent, deterministic, and reusable across queries while requiring only minimal changes to input parameters. SCOPE achieves state-of-the-art performance while lowering cost and latency. For example, with GPT-4o, it reaches 93.1% success on TravelPlanner, a 61.6% gain over the best baseline (CoT) while cutting inference cost by 1.4x and time by ~4.67x. Code is available at https://github.com/DerrickGXD/SCOPE.

==> Sections/baseline_prompts_full.tex <==
\subsection{Prompts for Tree-of-Thought (ToT)}
\needspace{6\baselineskip}

\begin{tcblisting}{title=Prompt for Expansion in Trip Planning, listing only, breakable}
Here is an example of query and full solution.

Example query : 
You plan to visit 10 European cities for 21 days in total. You only take direct flights to commute between cities. You plan to stay in Vienna for 3 days. You want to spend 5 days in Frankfurt. You want to spend 2 days in Oslo. You are going to attend a wedding in Oslo between day 20 and day 21. You want to spend 3 days in Prague. You would like to visit Valencia for 2 days. You want to meet a friend in Valencia between day 17 and day 18. You plan to stay in Dubrovnik for 2 days. You would like to visit Edinburgh for 5 days. From day 1 to day 5, there is a annual show you want to attend in Edinburgh. You plan to stay in London for 2 days. You plan to visit relatives in London between day 12 and day 13. You would like to visit Munich for 3 days. You would like to meet your friends at Munich between day 18 and day 20 to tour together. You would like to visit Budapest for 3 days.

Here are the cities that have direct flights:
Valencia and Munich, Vienna and Munich, Vienna and Valencia, London and Budapest, London and Oslo, Edinburgh and Budapest, Frankfurt and Budapest, Frankfurt and London, Prague and Oslo, Edinburgh and Oslo, Edinburgh and Munich, Prague and Munich, London and Prague, Edinburgh and London, Edinburgh and Frankfurt, Dubrovnik and Munich, Dubrovnik and Vienna, Munich and Oslo, Dubrovnik and Oslo, Budapest and Munich, Frankfurt and Prague, Vienna and London, Frankfurt and Vienna, Frankfurt and Oslo, Frankfurt and Munich, Vienna and Oslo, Vienna and Prague, Budapest and Oslo, Budapest and Prague, London and Valencia, London and Munich, Frankfurt and Dubrovnik, Prague and Valencia, Frankfurt and Valencia, Edinburgh and Prague, Vienna and Budapest.
Find a trip plan of visiting the cities for 21 days by taking direct flights to commute between them.

Example full solution ：
Here is the trip plan for visiting the 10 European cities for 21 days:

**Day 1-5:** Arriving in Edinburgh and visit Edinburgh for 5 days.
**Day 5:** Fly from Edinburgh to Frankfurt.
**Day 5-9:** Visit Frankfurt for 5 days.
**Day 9:** Fly from Frankfurt to Dubrovnik.
**Day 9-10:** Visit Dubrovnik for 2 days.
**Day 10:** Fly from Dubrovnik to Vienna.
**Day 10-12:** Visit Vienna for 3 days.
**Day 12:** Fly from Vienna to London.
**Day 12-13:** Visit London for 2 days.
**Day 13:** Fly from London to Budapest.
**Day 13-15:** Visit Budapest for 3 days.
**Day 15:** Fly from Budapest to Prague.
**Day 15-17:** Visit Prague for 3 days.
**Day 17:** Fly from Prague to Valencia.
**Day 17-18:** Visit Valencia for 2 days.
**Day 18:** Fly from Valencia to Munich.
**Day 18-20:** Visit Munich for 3 days.
**Day 20:** Fly from Munich to Oslo.
**Day 20-21:** Visit Oslo for 2 days.


You are a Tree-of-Thought (ToT) Agent. Given a query, a current state and the reasoning up to that state, you have to provide the next step for the current state.
In each step, you will output you next city you would like to visit and provide reasoning.

You must provide the reasoning of choosing this city. In every state, you choose N number of most possible cities (value of N is your choice), that you would like to visit from that current state.
If you are at first step, format is as below:
**Day 1-N:** Arriving in <first city> and visit <first city> for N days.

If you are at second step onwards, format is as below:
**Day X:** Fly from <current city> to <next city>.
**Day X-Y:** Visit <next city> for <N> days.

For example, the current state is:
Here is the trip plan for visiting the 10 European cities for 21 days:

**Day 1-5:** Arriving in Edinburgh and visit Edinburgh for 5 days.

Then, a possible example output of your next step is visiting Frankfurt:
**Day 5:** Fly from Edinburgh to Frankfurt.
**Day 5-9:** Visit Frankfurt for 5 days.



Your output format is a list as follows :
<start_of_output>
[
    {"next_step": <the output for your next step (choosing city 1)>, "reasoning": <your reasoning for choosing city 1>},
    {"next_step": <the output for your next step (choosing city 2)>, "reasoning": <your reasoning for choosing city 2>},
    ...
    {"next_step": <the output for your next step (choosing city N)>, "reasoning": <your reasoning for choosing city N>}
]
<end_of_output>

Query:
<query>

Current state:
<current_state>

Reasoning up to the state:
<reasoning_state>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Expansion in Meeting Planning, listing only, breakable}
Here is an example of query and full solution.

Example query : 
You are visiting San Francisco for the day and want to meet as many friends as possible. Solve the problem by considering various different schedules and picking the best one to optimize your goals.

Travel distances (in minutes):
Bayview to Alamo Square: 16.
Bayview to Union Square: 17.
Bayview to Golden Gate Park: 22.
Alamo Square to Bayview: 16.
Alamo Square to Union Square: 14.
Alamo Square to Golden Gate Park: 9.
Union Square to Bayview: 15.
Union Square to Alamo Square: 15.
Union Square to Golden Gate Park: 22.
Golden Gate Park to Bayview: 23.
Golden Gate Park to Alamo Square: 10.
Golden Gate Park to Union Square: 22.

CONSTRAINTS: You arrive at Bayview at 9:00AM. Ronald will be at Alamo Square from 8:30AM to 7:45PM. You'd like to meet Ronald for a minimum of 90 minutes. Richard will be at Union Square from 2:30PM to 9:45PM. You'd like to meet Richard for a minimum of 30 minutes. Kenneth will be at Golden Gate Park from 10:00AM to 3:15PM. You'd like to meet Kenneth for a minimum of 60 minutes.


Example full solution ：
SOLUTION:You start at Bayview at 9:00AM. You travel to Alamo Square in 16 minutes and arrive at 9:16AM. You meet Ronald for 90 minutes from 9:16AM to 10:46AM. You travel to Golden Gate Park in 9 minutes and arrive at 10:55AM. You meet Kenneth for 60 minutes from 10:55AM to 11:55AM. You travel to Union Square in 22 minutes and arrive at 12:17PM. You wait until 2:30PM. You meet Richard for 30 minutes from 2:30PM to 3:00PM.

You are a Tree-of-Thought (ToT) Agent. Given a query, a current state and the reasoning up to that state, you have to provide the next step for the current state.
In each step, you will output you next friend you would like to meet and provide reasoning.

You must provide the reasoning of choosing to meet this friend. In every state, you choose N number of most possible friends (value of N is your choice), that you would like to meet from that current state.
If you are at first step, format is as below:
SOLUTION:You start at <starting location> at <starting time>.

If you are at second step onwards, format is as below (If the person-to-meet's availability is not later than your arrival time):
You travel to <travel location> in <travel duration> and arrive at <arrival time>. You meet <person-to-meet> for <meeting duration> from <meeting start time> to <meeting end time>.

If you are at second step onwards, format is as below (If the person-to-meet's availability is later than your arrival time):
You travel to <travel location> in <travel duration> and arrive at <arrival time> You wait until <meeting start time>. You meet <person-to-meet> for <minimum meeting duration> from <meeting start time> to <meeting end time>.

For example, the current state is:
SOLUTION:You start at Bayview at 9:00AM.


Then, a possible example output of your next step is meeting Ronald:
You travel to Alamo Square in 16 minutes and arrive at 9:16AM. You meet Ronald for 90 minutes from 9:16AM to 10:46AM.


Your output format is a list as follows:
<start_of_output>
[
    {"next_step": <the output for your next friend to meet (choosing friend 1)>, "reasoning": <your reasoning for choosing friend 1>},
    {"next_step": <the output for your next friend to meet (choosing friend 2)>, "reasoning": <your reasoning for choosing friend 2>},
    ...
    {"next_step": <the output for your next friend to meet (choosing friend N)>, "reasoning": <your reasoning for choosing friend N>}
]
<end_of_output>

You must follow this output format and wrap your output with <start_of_output> and <end_of_output> tag. Do not output anything else.

Query:
<query>

Current state:
<current_state>

Reasoning up to the state:
<reasoning_state>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Expansion in Travel Planner, listing only, breakable}
"You are a proficient planner. Based on the provided information and query, please give me a detailed plan, including specifics such as flight numbers (e.g., F0123456), restaurant names, and accommodation names. Note that all the information in your plan should be derived from the provided data. You must adhere to the format given in the example. Additionally, all details should align with commonsense. The symbol '-' indicates that information is unnecessary. For example, in the provided sample, you do not need to plan after returning to the departure city. When you travel to two cities in one day, you should note it in the 'Current City' section as in the example (i.e., from A to B).

The rules of travelling is as follows :
1. Travel to another location in odd number day and staying in the same city at even number.
2. When staying in each city, an accommodation, an attractions and 3 restaurants are required. You are required to stay in the same accommodation in the city for two days. 
3. For the last day, you are required to travel back to the starting location.
4. If no number of people are mentioned in the query, you should assume only 1 person is travelling.
5. You should assume if the accommodation room maximum capacity exceeds the number of people, the user will still consider staying in the accommodation. However, the user will book multiple rooms of the same accommodation.
6. However, if the accommodation room minimum nights exceed the query's minimum nights, the plan will fail.
7. If user is taking flight, the user should buy tickets for everyone in the trip. The cost for flight is per ticket.
8. You should also assume a self-driving car can fit 5 people while a taxi car can fit 4 people. If the number of people in the trip exceeds the capacity of vehicle (for example taxi), you assume the user will book multiple vehicles (for example multiple taxis).
9. You are not allowed to have 'self-driving and flight' or 'self-driving and taxi' in a trip. 
10. You are not allowed to have repeated restaurants throughout the trip. 

Here is an example of query and full solution.

Example query : 
Can you help with generating a 7-day travel plan for a party of 5? We're setting off from Indianapolis and planning to explore 3 cities in Colorado from March 11th to March 17th, 2022. We have a budget of $15,100 for this trip. We'll be bringing our pets, so pet-friendly accommodations are a must. We're also hoping to find places that offer Mexican, Italian, Mediterranean, and Indian cuisines. Entire rooms for accommodations would be ideal.

Example full solution ：
Travel Plan:
Day 1:
Current City: from Indianapolis to Grand Junction
Transportation: Taxi, from Indianapolis to Grand Junction
Breakfast: -
Attraction: -
Lunch: -
Dinner: -
Accommodation: NYC Apartment near Central Park!, Grand Junction

Day 2:
Current City: Grand Junction
Transportation: -
Breakfast: Austin's BBQ and Oyster Bar, Grand Junction
Attraction: Museum of the West, Museums of Western Colorado, Grand Junction
Lunch: Punjab Da Pind, Grand Junction
Dinner: Cha Bar, Grand Junction
Accommodation: NYC Apartment near Central Park!, Grand Junction

Day 3:
Current City: from Grand Junction to Alamosa
Transportation: Taxi, from Grand Junction to Alamosa
Breakfast: -
Attraction: -
Lunch: -
Dinner: -
Accommodation: Private & Quaint West Village Gem!, Alamosa

Day 4:
Current City: Alamosa
Transportation: -
Breakfast: Good Luck Cafe, Alamosa
Attraction: San Luis Valley Museum | Alamosa, Alamosa
Lunch: Lights Camera Action - Air Bar, Alamosa
Dinner: Street Foods by Punjab Grill, Alamosa
Accommodation: Private & Quaint West Village Gem!, Alamosa

Day 5:
Current City: from Alamosa to Denver
Transportation: Flight Number: F3837896, from Alamosa to Denver
Breakfast: -
Attraction: -
Lunch: -
Dinner: -
Accommodation: GORGEOUS Newly-Renovated 2-BR Flat, Denver

Day 6:
Current City: Denver
Transportation: -
Breakfast: The Urban Socialite, Denver
Attraction: Denver Zoo, Denver
Lunch: Woods Spice, Denver
Dinner: Radhika Sweets, Denver
Accommodation: GORGEOUS Newly-Renovated 2-BR Flat, Denver

Day 7:
Current City: from Denver to Indianapolis
Transportation: Flight Number: F3910575, from Denver to Indianapolis
Breakfast: -
Attraction: -
Lunch: -
Dinner:-
Accommodation: -


Instead of providing the full solution, you are required to solve it using Tree-of-Thought (ToT). Given a query, reference information, a current state and the reasoning up to that state, you have to provide the next step for the current state.
In each step, you will output "Current City", "Transportation", "Breakfast", "Attraction", "Lunch", "Dinner", "Accommodation" and provide reasoning..

You must provide the reasoning of choosing these options. In every state, you choose N number of most possible set of plans (value of N is your choice), that you would like to fill in the plan for next day.

Your output format is as below (The output is in string of multiple lines, not JSON):
Day N:
Current City: <fill in your option. "-" for None>
Transportation: <fill in your option. "-" for None>
Breakfast: <fill in your option. "-" for None>
Attraction: <fill in your option. "-" for None>
Lunch: <fill in your option. "-" for None>
Dinner: <fill in your option. "-" for None>
Accommodation: <fill in your option. "-" for None>


For example, the current state is:
Travel Plan:
Day 1:
Current City: from Indianapolis to Grand Junction
Transportation: Taxi, from Indianapolis to Grand Junction
Breakfast: -
Attraction: -
Lunch: -
Dinner: -
Accommodation: NYC Apartment near Central Park!, Grand Junction


Then, a possible example output of your next step:
Day 2:
Current City: Grand Junction
Transportation: -
Breakfast: Austin's BBQ and Oyster Bar, Grand Junction
Attraction: Museum of the West, Museums of Western Colorado, Grand Junction
Lunch: Punjab Da Pind, Grand Junction
Dinner: Cha Bar, Grand Junction
Accommodation: NYC Apartment near Central Park!, Grand Junction

You must follow the output format given to you.
Your output format is a list as follows :
<start_of_output>
[
    {"next_step": <the output for your next step (next day's plan). Output is in string format. Please do not output JSON>, "reasoning": <your reasoning for choosing this plan>},
    {"next_step": <the output for your next step (next day's plan). Output is in string format. Please do not output JSON>, "reasoning": <your reasoning for choosing this plan>},
    ...
    {"next_step": <the output for your next step (next day's plan). Output is in string format. Please do not output JSON>, "reasoning": <your reasoning for choosing this plan>}
]
<end_of_output>

Query:
<query>

Reference information:
<text>

Current state:
<current_state>

Reasoning up to the state:
<reasoning_state>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Evaluation in Natural Plan, listing only, breakable}
You are a Tree-of-Thought (ToT) Evaluator. Given a query, list of current states and reasoning for each state, you have to evaluate and provide score for each state of how likely each state will lead to correct solution.
Your score should be between 1 and 10. Only integer is allowed.
In your output, you must copy each state and reasoning exactly as the input, do not change any words.
You must ensure the score for each output are different. You are not allowed to provide same score for different output.

The current states and reasoning is given in such format:
[
    {"current_state": <current state>, "reasoning": <reasoning for the state>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>}
]

Your output format is a list as follows :
<start_of_output>
[
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>}
]
<end_of_output>

Query:
<query>

Current states and reasoning:
<current_state>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Evaluation in Travel Planner, listing only, breakable}
You are a Tree-of-Thought (ToT) Evaluator. Given a query, list of current states and reasoning for each state, you have to evaluate and provide score for each state of how likely each state will lead to correct solution.
Your score should be between 1 and 10. Only integer is allowed.
In your output, you must copy each state and reasoning exactly as the input, do not change any words.
You must ensure the score for each output are different. You are not allowed to provide same score for different output.

You must consider these rules of travelling when giving your scores :
1. Travel to another location in odd number day and staying in the same city at even number.
2. When staying in each city, an accommodation, an attractions and 3 restaurants are required. You are required to stay in the same accommodation in the city for two days. 
3. For the last day, you are required to travel back to the starting location.
4. If no number of people are mentioned in the query, you should assume only 1 person is travelling.
5. You should assume if the accommodation room maximum capacity exceeds the number of people, the user will still consider staying in the accommodation. However, the user will book multiple rooms of the same accommodation.
6. However, if the accommodation room minimum nights exceed the query's minimum nights, the plan will fail.
7. If user is taking flight, the user should buy tickets for everyone in the trip. The cost for flight is per ticket.
8. You should also assume a self-driving car can fit 5 people while a taxi car can fit 4 people. If the number of people in the trip exceeds the capacity of vehicle (for example taxi), you assume the user will book multiple vehicles (for example multiple taxis).
9. You are not allowed to have 'self-driving and flight' or 'self-driving and taxi' in a trip. 
10. You are not allowed to have repeated restaurants throughout the trip. 

The current states and reasoning is given in such format:
[
    {"current_state": <current state>, "reasoning": <reasoning for the state>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>}
]

Your output format is a list as follows :
<start_of_output>
[
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>},
    {"current_state": <current state>, "reasoning": <reasoning for the state>, "score": <integer between 1 and 10>}
]
<end_of_output>

Query:
<query>

Current states and reasoning:
<current_state>

\end{tcblisting}

\newpage

\subsection{Prompts for Thought of Search (ToS)}
\needspace{6\baselineskip}

\begin{tcblisting}{title=Prompt for Introduction, listing only, breakable}
You are a task description agent. There is a task called <task>. You are given an example query and answer of the task. Using this query and answer, you must provide a detailed description of task.
You must also provide any assumptions or constraints that are not explicit in the query. Your assumptions and constraints must be general so that can be applied on other queries of <task>.
Finally, you must also mention how a state is represented. You should also describe how to transition from one state to another and what is the ending state.
Lastly, you list out the conditions where a state has met the goal by writing the list of conditions after.

Your output format is as below:
Description of <task>:
<your description of task>

Description of how to transition from one state to another and ending state:
<the description>

List of conditions where a state has met the goal:
1. <Condition 1>
...
N. <Condition N>

Here is an example task called 24 Game and here is the example output description :

The 24 Game is a mathematical card game where the objective is to manipulate four integers so that the final result equals 24. The game begins with a list of four numbers, and the player must use each number exactly once, applying any combination of addition, subtraction, multiplication, or division to obtain 24.
A state is represented as a list of numbers (of length four or fewer).


An example query of the task :
<task_query>

An example answer of the task :
<task_answer>

Your output :
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Evaluation in Natural Plan, listing only, breakable}
You are a function generator agent. There is a task called <task>.

First of all, you must define the state. To do that, you provide the state from the given example query.

Write a Python function called 'successor_states(state)' that generates all valid successor states for the <task>.

Then, write a Python function called 'is_goal(state)' that tests whether a state is a goal state. 

Then, write a Python function called 'convert_state_to_nl(state)' that convert the goal state to NL that shares the same format as the example answer.
Hence, you must ensure the goal state contain the sufficient information be converted to NL.

Please do not include any example usage or print anything in your code. Ensure your code is written within the given wrapper. Please don't include ```python and ``` wrapper in your output.
Please do not hardcode any fixed values in any functions that cannot be applied to other queries of <task>.


The task description of <task> is as follows :
<task_description>

An example query of the task :
<task_query>

An example answer of the task :
<task_answer>

Your output format is as follows :

State structure:
<start_of_JSON>
<your state given the example query>
<end_of_JSON>

Output code for successor_states:
<start_of_code>
<your code. Please do not hardcode any fixed values in any functions that cannot be applied to other queries.>
<end_of_code>

Output code for is_goal:
<start_of_code>
<your code. Please do not hardcode any fixed values in any functions that cannot be applied to other queries.>
<end_of_code>

Output code for convert_state_to_nl:
<start_of_code>
<your code. Remember, the function output must share the same format as the answer of the task.>
<end_of_code>

\end{tcblisting}


==> Sections/output_full.tex <==
\subsection{Output of Agents for Trip Planning}

\begin{tcblisting}{title=Output of Solution Agent, listing only, breakable}
<start_of_structured_output>
{
    "solutions": [
        {"city": "Edinburgh", "days": [1, 2, 3, 4, 5]},
        {"city": "Frankfurt", "days": [5, 6, 7, 8, 9]},
        {"city": "Dubrovnik", "days": [9, 10]},
        {"city": "Vienna", "days": [10, 11, 12]},
        {"city": "London", "days": [12, 13]},
        {"city": "Budapest", "days": [13, 14, 15]},
        {"city": "Prague", "days": [15, 16, 17]},
        {"city": "Valencia", "days": [17, 18]},
        {"city": "Munich", "days": [18, 19, 20]},
        {"city": "Oslo", "days": [20, 21]}
    ],
    "solutions_description": "The 'solutions' key contains a list of dictionaries, each representing a city visit during the trip. Each dictionary has two keys: 'city' and 'days'. The 'city' key holds the name of the city being visited, and the 'days' key contains a list of integers representing the days of the trip spent in that city."
}
<end_of_structured_output>
\end{tcblisting}


\begin{tcblisting}{title=Output of Planner Agent, listing only, breakable}
<start_of_COT>
Informations that are essential for generating combinations :
- List of cities to visit.
- Total number of days for the trip.
- Direct flight connections between cities.

Constraints that are essential for filtering plans :
- Specific number of days to stay in each city.
- Specific days to be in certain cities for events or meetings.
- Total trip duration must be exactly 21 days.
- Must only use direct flights between cities.
<end_of_COT>

<start_of_structured_output>
{
    "combinations": {
        "cities": ["Edinburgh", "Frankfurt", "Dubrovnik", "Vienna", "London", "Budapest", "Prague", "Valencia", "Munich", "Oslo"],
        "total_days": 21,
        "direct_flights": [
            ["Valencia", "Munich"], ["Vienna", "Munich"], ["Vienna", "Valencia"], ["London", "Budapest"],
            ["London", "Oslo"], ["Edinburgh", "Budapest"], ["Frankfurt", "Budapest"], ["Frankfurt", "London"],
            ["Prague", "Oslo"], ["Edinburgh", "Oslo"], ["Edinburgh", "Munich"], ["Prague", "Munich"],
            ["London", "Prague"], ["Edinburgh", "London"], ["Edinburgh", "Frankfurt"], ["Dubrovnik", "Munich"],
            ["Dubrovnik", "Vienna"], ["Munich", "Oslo"], ["Dubrovnik", "Oslo"], ["Budapest", "Munich"],
            ["Frankfurt", "Prague"], ["Vienna", "London"], ["Frankfurt", "Vienna"], ["Frankfurt", "Oslo"],
            ["Frankfurt", "Munich"], ["Vienna", "Oslo"], ["Vienna", "Prague"], ["Budapest", "Oslo"],
            ["Budapest", "Prague"], ["London", "Valencia"], ["London", "Munich"], ["Frankfurt", "Dubrovnik"],
            ["Prague", "Valencia"], ["Frankfurt", "Valencia"], ["Edinburgh", "Prague"], ["Vienna", "Budapest"]
        ]
    },
    "constraints": {
        "city_stays": {
            "Edinburgh": 5,
            "Frankfurt": 5,
            "Dubrovnik": 2,
            "Vienna": 3,
            "London": 2,
            "Budapest": 3,
            "Prague": 3,
            "Valencia": 2,
            "Munich": 3,
            "Oslo": 2
        },
        "specific_days": {
            "Edinburgh": [1, 5],
            "Oslo": [20, 21],
            "Valencia": [17, 18],
            "London": [12, 13],
            "Munich": [18, 20]
        }
    },
    "combinations_description": "The 'combinations' key contains the parameters for generating possible travel plans. 'cities' is a list of cities to visit, 'total_days' is the total number of days for the trip, and 'direct_flights' is a list of pairs of cities that have direct flights between them.",
    "constraints_description": "The 'constraints' key contains the conditions that must be met for a valid travel plan. 'city_stays' specifies the number of days to stay in each city, and 'specific_days' specifies the exact days certain cities must be visited for events or meetings."
}
<end_of_structured_output>

<start_of_planning>
{
    "Input Agent": "Identify the set of cities to visit, the total number of days for the trip, and the direct flight connections between cities. Also, identify the constraints such as the number of days to stay in each city and specific days to be in certain cities for events or meetings.",
    "Combination Function Generator Agent": "Create a function combinations_func() that takes 'cities', 'total_days', and 'direct_flights' as input. Generate all possible sequences of city visits that fit within the total days and only use direct flights.",
    "Solution Function Generator Agent": "Create a function plan_func() that takes 'city_stays' and 'specific_days' as constraints, along with the list of possible plans from combinations_func(). Filter the plans to find one that satisfies all constraints, ensuring the total trip duration is exactly 21 days and all specific day requirements are met."
}
<end_of_planning>
\end{tcblisting}

\begin{tcblisting}{title=Output of Combination Function Generator Agent, listing only, breakable}
<start_of_COT>
To solve this problem, we need to generate all possible sequences of city visits that fit within the total days and only use direct flights. Here's the step-by-step thought process:

1. **Input Parsing**: We will extract the list of cities, direct flights, and city stays from the input dictionary.

2. **Graph Representation**: We will represent the direct flights as a graph where each city is a node and each direct flight is an edge. This will help us in determining valid paths.

3. **Permutations and Combinations**: We will use permutations to generate possible sequences of city visits. However, we need to ensure that each sequence is valid in terms of direct flights and total days.

4. **Validation of Sequences**:
   - For each permutation of cities, we will check if there is a direct flight between consecutive cities.
   - We will also calculate the total days required for each sequence by summing up the days required for each city stay.
   - If the total days exceed the allowed days, the sequence is invalid.

5. **Output Format**: For each valid sequence, we will create a list of dictionaries where each dictionary contains the city name and the days spent in that city. The days will be represented as a list of integers.

6. **Return the Result**: Finally, we will return a list of all valid sequences in the specified format.

By following these steps, we ensure that the function generates all possible valid travel plans according to the given constraints.
<end_of_COT>

<start_of_code>
from itertools import permutations

def combinations_func(data):
    cities = data['cities']
    direct_flights = data['direct_flights']
    city_stays = data['city_stays']
    
    # Create a set of direct flights for quick lookup
    flight_set = set(tuple(flight) for flight in direct_flights)
    
    # Calculate total days available
    total_days = sum(city_stays.values())
    
    # List to store all valid plans
    valid_plans = []
    
    # Generate all permutations of cities
    for perm in permutations(cities):
        current_day = 1
        valid = True
        plan = []
        
        for i in range(len(perm)):
            city = perm[i]
            stay_days = city_stays[city]
            
            # Check if the current city can be reached from the previous city
            if i > 0:
                prev_city = perm[i - 1]
                if (prev_city, city) not in flight_set:
                    valid = False
                    break
            
            # Add the city and its stay days to the plan
            plan.append({
                "city": city,
                "days": list(range(current_day, current_day + stay_days))
            })
            
            # Update the current day
            current_day += stay_days
            
            # Check if the total days exceed the allowed days
            if current_day > total_days + 1:
                valid = False
                break
        
        # If the plan is valid, add it to the list of valid plans
        if valid:
            valid_plans.append(plan)
    
    return valid_plans
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Solution Function Generator Agent, listing only, breakable}
<start_of_COT>
To solve this problem, we need to filter the list of plans based on the constraints provided. The constraints specify certain days that specific cities must be visited. Our task is to find a plan that satisfies all these constraints.

1. **Understand the Input Format**:
   - Each plan is a list of dictionaries, where each dictionary represents a city visit with the city name and the days spent there.
   - Constraints are given in a dictionary format, where 'specific_days' specifies the exact days certain cities must be visited.

2. **Plan the Function**:
   - Iterate over each plan in the 'data' list.
   - For each plan, check if it satisfies all the constraints specified in 'specific_days'.
   - For each city in 'specific_days', ensure that the city is visited on all the required days in the plan.
   - If a plan satisfies all constraints, return that plan.

3. **Implementation Steps**:
   - Loop through each plan in the data.
   - For each plan, loop through each city in the 'specific_days' constraints.
   - Check if the city is present in the plan and if the days match the required days.
   - If all constraints are satisfied for a plan, return that plan.

4. **Edge Cases**:
   - If no plan satisfies the constraints, the function should handle this gracefully (though the problem does not specify what to do in this case, we assume at least one valid plan exists).

By following these steps, we can ensure that the function correctly filters and returns a plan that meets all the specified constraints.
<end_of_COT>

<start_of_code>
def plan_func(data, constraints):
    specific_days = constraints.get('specific_days', {})
    
    for plan in data:
        all_constraints_met = True
        
        for city, required_days in specific_days.items():
            city_found = False
            
            for visit in plan:
                if visit['city'] == city:
                    city_days = set(visit['days'])
                    if all(day in city_days for day in required_days):
                        city_found = True
                        break
            
            if not city_found:
                all_constraints_met = False
                break
        
        if all_constraints_met:
            return plan
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Deliverer Function Generator Agent, listing only, breakable}
<start_of_COT>
1. The few-shot example solution begins with a heading that summarizes the trip plan, mentioning the number of cities and days. The format is: "Here is the trip plan for visiting the X European cities for Y days:".
2. The output then details each city visit and the transitions between cities. Each city visit is described with the format: "**Day X-Y:** Visit [City] for Z days.".
3. Transitions between cities are described with the format: "**Day X:** Fly from [City1] to [City2].".
4. The function needs to iterate through the list of city visits, keeping track of the current day and ensuring that transitions and visits are formatted correctly.
5. The function should handle overlapping days correctly, ensuring that transitions are noted on the correct day.

To design the function:
- Start by calculating the total number of cities and days.
- Initialize a string with the heading.
- Iterate through the list of city visits, formatting each visit and transition according to the example.
- Keep track of the current day and adjust for overlaps in days between cities.
- Append each formatted string to the result.
- Return the complete formatted string as the output.
<end_of_COT>

<start_of_code>
def deliver_func(data):
    num_cities = len(data)
    total_days = max(day for city in data for day in city['days'])
    
    result = f"Here is the trip plan for visiting the {num_cities} European cities for {total_days} days:\n\n"
    
    current_day = 1
    for i, visit in enumerate(data):
        city = visit['city']
        days = visit['days']
        start_day = days[0]
        end_day = days[-1]
        visit_days = end_day - start_day + 1
        
        if start_day == current_day:
            result += f"**Day {start_day}-{end_day}:** Visit {city} for {visit_days} days.\n"
        else:
            result += f"**Day {start_day}:** Fly from {data[i-1]['city']} to {city}.\n"
            result += f"**Day {start_day}-{end_day}:** Visit {city} for {visit_days} days.\n"
        
        current_day = end_day + 1
    
    return result
<end_of_code>
\end{tcblisting}

\clearpage

\subsection{Output of Agents for Meeting Planning}
\begin{tcblisting}{title=Output of Solution Agent, listing only, breakable}
<start_of_structured_output>
{
    "solutions": {
        "initial_starting_point": {
            "location": "Marina District",
            "start_time": "9:00AM"
        },
        "meetings": [
            {
                "person": "Jessica",
                "meeting_start_time": "2:30PM",
                "meeting_end_time": "3:45PM",
                "meeting_location": "Alamo Square",
                "travel_duration_minutes": 15,
                "waiting_time_minutes": 315
            },
            {
                "person": "Ronald",
                "meeting_start_time": "4:04PM",
                "meeting_end_time": "5:04PM",
                "meeting_location": "Fisherman's Wharf",
                "travel_duration_minutes": 19,
                "waiting_time_minutes": 0
            },
            {
                "person": "Mary",
                "meeting_start_time": "7:00PM",
                "meeting_end_time": "7:45PM",
                "meeting_location": "Union Square",
                "travel_duration_minutes": 13,
                "waiting_time_minutes": 103
            }
        ]
    },
    "solutions_description": "The 'solutions' key contains the structured details of the schedule. The 'initial_starting_point' key provides the starting location and time. The 'meetings' key is a list of meetings, where each meeting includes the following details: 'person' (the name of the person to meet), 'meeting_start_time' (the time the meeting starts), 'meeting_end_time' (the time the meeting ends), 'meeting_location' (the location of the meeting), 'travel_duration_minutes' (the time in minutes it takes to travel from the previous location to the meeting location), and 'waiting_time_minutes' (the time in minutes spent waiting due to arriving earlier than the person's availability)."
}
<end_of_structured_output>
\end{tcblisting}


\begin{tcblisting}{title=Output of Planner Agent, listing only, breakable}
<start_of_COT>
Informations that are essential for generating combinations :
- The starting location and time of the schedule.
- The list of people to meet, including their names and the locations where they will be available.
- The travel distances (in minutes) between all possible locations.
- The availability windows for each person (start and end times).

Constraints that are essential for filtering plans :
- The minimum meeting duration required for each person.
- The availability windows for each person (start and end times).
- The travel time between locations must be accounted for to ensure the schedule is feasible.
- The schedule must start at the specified starting location and time.
<end_of_COT>

<start_of_structured_output>
{
    "parameters": {
        "starting_point": {
            "location": "Marina District",
            "start_time": "09:00"
        },
        "people": [
            {
                "name": "Jessica",
                "location": "Alamo Square",
                "availability_start_time": "14:30",
                "availability_end_time": "20:15",
                "minimum_meeting_duration_minutes": 75
            },
            {
                "name": "Ronald",
                "location": "Fisherman's Wharf",
                "availability_start_time": "15:15",
                "availability_end_time": "18:30",
                "minimum_meeting_duration_minutes": 60
            },
            {
                "name": "Mary",
                "location": "Union Square",
                "availability_start_time": "19:00",
                "availability_end_time": "22:00",
                "minimum_meeting_duration_minutes": 45
            }
        ],
        "travel_times": {
            "Marina District": {
                "Alamo Square": 15,
                "Fisherman's Wharf": 10,
                "Union Square": 16
            },
            "Alamo Square": {
                "Marina District": 15,
                "Fisherman's Wharf": 19,
                "Union Square": 14
            },
            "Fisherman's Wharf": {
                "Marina District": 9,
                "Alamo Square": 20,
                "Union Square": 13
            },
            "Union Square": {
                "Marina District": 18,
                "Alamo Square": 15,
                "Fisherman's Wharf": 15
            }
        }
    },
    "parameters_description": "The 'parameters' key contains the details required to generate combinations. The 'starting_point' key specifies the initial location and time. The 'people' key is a list of individuals to meet, where each entry includes the person's name, meeting location, availability window (start and end times), and the minimum meeting duration in minutes. The 'travel_times' key provides a nested dictionary of travel durations (in minutes) between all possible locations."
}
<end_of_structured_output>

<start_of_planning>
{
    "Input Agent": "The Input Agent should identify the starting location and time, the list of people to meet (including their names, locations, availability windows, and minimum meeting durations), and the travel times between all locations. The output should include these details under the keys 'combinations' (for generating plans), 'constraints' (for filtering plans), and 'solutions' (for the final schedule).",
    "Combination Function Generator Agent": "The Combination Function Generator Agent should create a function called combinations_func() that takes the 'parameters' key as input. The function should generate all possible schedules by considering permutations of meeting orders and calculating the travel times and waiting times for each schedule. Each plan should include the starting point, the sequence of meetings (with details such as person, meeting location, travel duration, and waiting time), and the total time spent.",
    "Solution Function Generator Agent": "The Solution Function Generator Agent should create a function called plan_func() that takes the 'constraints' and the output of combinations_func() as input. Since this is an optimization problem, the function should filter out plans that do not meet the constraints (e.g., minimum meeting durations, availability windows, and travel feasibility) and return the plan that maximizes the number of meetings while minimizing total travel and waiting time."
}
<end_of_planning>
\end{tcblisting}

\begin{tcblisting}{title=Output of Combination Function Generator Agent, listing only, breakable}
<start_of_COT>

To solve this problem, we need to generate all possible schedules for meeting people based on the input data. Here's the step-by-step thought process:

1. **Understand the Input**: The input contains:
   - A starting point with a location and start time.
   - A list of people to meet, each with a name, meeting location, availability window, and minimum meeting duration.
   - A dictionary of travel times between locations.

2. **Understand the Output**: The output should be a list of possible schedules. Each schedule includes:
   - The initial starting point (location and time).
   - A sequence of meetings, where each meeting includes:
     - The person's name.
     - Meeting start and end times.
     - Meeting location.
     - Travel duration from the previous location.
     - Waiting time before the meeting starts.

3. **Generate All Permutations**: Since the order of meetings matters, we need to generate all permutations of the people to meet. This will allow us to explore all possible meeting orders.

4. **Calculate Travel and Waiting Times**:
   - For each permutation, calculate the travel time between locations using the `travel_times` dictionary.
   - Check if the meeting can start within the person's availability window. If the arrival time is earlier than the availability start time, calculate the waiting time. If the arrival time is later than the availability end time, skip this meeting.
   - Ensure the meeting duration is at least the minimum required duration.

5. **Build the Schedule**:
   - Start from the initial location and time.
   - For each person in the permutation, calculate the meeting details (start time, end time, travel duration, waiting time) and add them to the schedule.
   - If a meeting cannot be scheduled due to time constraints, skip it and continue with the next person.

6. **Store the Results**: For each valid schedule, store the details in the required format.

7. **Return the Results**: Return a list of all possible schedules.

The two helper functions (`hhmm_to_minutes` and `minutes_to_hhmm`) will be used to handle time calculations. The main function will use these to convert times to minutes for easier calculations and then back to HH:MM format for the output.

<end_of_COT>

<start_of_code>
from itertools import permutations

# Convert HH:MM to minutes
def hhmm_to_minutes(time_str):
    hours, minutes = map(int, time_str.split(":"))
    return hours * 60 + minutes

# Convert minutes to HH:MM
def minutes_to_hhmm(total_minutes):
    hours = total_minutes // 60
    minutes = total_minutes % 60
    return f"{hours:02d}:{minutes:02d}"

def combinations_func(data):
    starting_point = data["starting_point"]
    people = data["people"]
    travel_times = data["travel_times"]

    start_location = starting_point["location"]
    start_time = hhmm_to_minutes(starting_point["start_time"])

    # Generate all permutations of people
    all_permutations = list(permutations(people))

    solutions = []

    # Iterate through each permutation
    for perm in all_permutations:
        current_time = start_time
        current_location = start_location
        schedule = {
            "initial_starting_point": {
                "location": start_location,
                "start_time": minutes_to_hhmm(start_time)
            },
            "meetings": []
        }
        valid_schedule = True

        # Iterate through each person in the permutation
        for person in perm:
            person_name = person["name"]
            meeting_location = person["location"]
            availability_start = hhmm_to_minutes(person["availability_start_time"])
            availability_end = hhmm_to_minutes(person["availability_end_time"])
            minimum_meeting_duration = person["minimum_meeting_duration_minutes"]

            # Calculate travel time to the meeting location
            travel_duration = travel_times[current_location][meeting_location]
            arrival_time = current_time + travel_duration

            # Check if the meeting can be scheduled
            if arrival_time > availability_end:
                valid_schedule = False
                break  # Skip this permutation if the meeting cannot be scheduled

            # Calculate waiting time
            waiting_time = max(0, availability_start - arrival_time)

            # Calculate meeting start and end times
            meeting_start_time = max(arrival_time, availability_start)
            meeting_end_time = meeting_start_time + minimum_meeting_duration

            # Check if the meeting ends within the availability window
            if meeting_end_time > availability_end:
                valid_schedule = False
                break  # Skip this permutation if the meeting cannot be scheduled

            # Add the meeting to the schedule
            schedule["meetings"].append({
                "person": person_name,
                "meeting_start_time": minutes_to_hhmm(meeting_start_time),
                "meeting_end_time": minutes_to_hhmm(meeting_end_time),
                "meeting_location": meeting_location,
                "travel_duration_minutes": travel_duration,
                "waiting_time_minutes": waiting_time
            })

            # Update current time and location
            current_time = meeting_end_time
            current_location = meeting_location

        # Add the schedule to the solutions if it's valid
        if valid_schedule:
            solutions.append(schedule)

    return solutions
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Solution Function Generator Agent, listing only, breakable}
<start_of_COT>
To solve this problem, we need to filter and evaluate the plans based on the given constraints. The goal is to find the plan that maximizes the number of meetings while minimizing total travel and waiting time. Here's the step-by-step approach:

1. **Filter Plans Based on Constraints**:
   - Ensure that the initial starting point in the plan matches the `starting_point` in the constraints.
   - For each meeting in the plan, check if:
     - The meeting's start and end times fall within the person's availability window.
     - The meeting duration meets or exceeds the minimum meeting duration specified in the constraints.
     - The travel time between meetings is feasible based on the `travel_times` provided in the constraints.

2. **Evaluate Plans**:
   - For each valid plan, calculate:
     - The total number of meetings.
     - The total travel time across all meetings.
     - The total waiting time across all meetings.
   - Use these metrics to rank the plans. The primary goal is to maximize the number of meetings. If there are ties, prioritize plans with lower total travel time and then lower total waiting time.

3. **Return the Best Plan**:
   - After evaluating all valid plans, return the one that best meets the optimization criteria.

4. **Implementation Details**:
   - Parse the time strings into comparable datetime objects for accurate calculations.
   - Use the `travel_times` dictionary to validate travel feasibility between locations.
   - Ensure that all constraints are respected when filtering and evaluating plans.

<end_of_COT>

<start_of_code>
from datetime import datetime, timedelta

def parse_time(time_str):
    """Helper function to parse time strings into datetime objects."""
    return datetime.strptime(time_str, "%I:%M%p")

def plan_func(data, constraints):
    def is_meeting_valid(meeting, person_constraints, prev_location, prev_end_time):
        """Check if a meeting is valid based on constraints."""
        # Check if the meeting is with the correct person
        if meeting["person"] != person_constraints["name"]:
            return False
        
        # Check if the meeting location matches
        if meeting["meeting_location"] != person_constraints["location"]:
            return False
        
        # Check if the meeting duration meets the minimum requirement
        meeting_start = parse_time(meeting["meeting_start_time"])
        meeting_end = parse_time(meeting["meeting_end_time"])
        meeting_duration = (meeting_end - meeting_start).total_seconds() / 60
        if meeting_duration < person_constraints["minimum_meeting_duration_minutes"]:
            return False
        
        # Check if the meeting falls within the person's availability window
        availability_start = parse_time(person_constraints["availability_start_time"])
        availability_end = parse_time(person_constraints["availability_end_time"])
        if not (availability_start <= meeting_start and meeting_end <= availability_end):
            return False
        
        # Check if travel time from the previous location is feasible
        travel_time = constraints["travel_times"][prev_location][meeting["meeting_location"]]
        if prev_end_time + timedelta(minutes=travel_time) > meeting_start:
            return False
        
        return True

    def evaluate_plan(plan):
        """Evaluate a plan based on the number of meetings, total travel time, and waiting time."""
        total_meetings = len(plan["meetings"])
        total_travel_time = sum(meeting["travel_duration_minutes"] for meeting in plan["meetings"])
        total_waiting_time = sum(meeting["waiting_time_minutes"] for meeting in plan["meetings"])
        return total_meetings, total_travel_time, total_waiting_time

    # Filter and evaluate plans
    valid_plans = []
    for plan in data:
        # Check if the initial starting point matches
        if plan["initial_starting_point"]["location"] != constraints["starting_point"]["location"]:
            continue
        
        # Validate each meeting in the plan
        valid = True
        prev_location = plan["initial_starting_point"]["location"]
        prev_end_time = parse_time(plan["initial_starting_point"]["start_time"])
        for meeting in plan["meetings"]:
            # Find the corresponding person constraints
            person_constraints = next((p for p in constraints["people"] if p["name"] == meeting["person"]), None)
            if not person_constraints or not is_meeting_valid(meeting, person_constraints, prev_location, prev_end_time):
                valid = False
                break
            # Update previous location and end time
            prev_location = meeting["meeting_location"]
            prev_end_time = parse_time(meeting["meeting_end_time"])
        
        if valid:
            valid_plans.append(plan)
    
    # Rank the valid plans
    best_plan = None
    best_score = None
    for plan in valid_plans:
        total_meetings, total_travel_time, total_waiting_time = evaluate_plan(plan)
        score = (-total_meetings, total_travel_time, total_waiting_time)  # Negative meetings for maximization
        if best_score is None or score < best_score:
            best_plan = plan
            best_score = score
    
    return best_plan
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Deliverer Function Generator Agent, listing only, breakable}
<start_of_COT>
1. The few-shot example solution does not contain any heading. It is a narrative description of the itinerary, starting from the initial location and time, followed by a sequence of travel and meeting events. Each event is described in a sentence that includes the action (travel, wait, meet), the location, the duration, and the time.

2. To design the function, I will:
   - Extract the initial start location and time.
   - Iterate through each meeting in the 'meetings' list.
   - Calculate the arrival time at each meeting location by adding the travel duration to the previous event's end time.
   - If there is waiting time, include a statement about waiting until the meeting start time.
   - Describe the meeting duration and times.
   - Ensure the output is a continuous narrative that matches the example format.
   - Use time calculations to handle AM/PM conversions and ensure correct time formatting.
<end_of_COT>

<start_of_code>
from datetime import datetime, timedelta

def deliver_func(data):
    def parse_time(time_str):
        return datetime.strptime(time_str, "%I:%M%p")
    
    def format_time(time_obj):
        return time_obj.strftime("%I:%M%p").lstrip("0").replace(" 0", " ")
    
    itinerary = []
    current_time = parse_time(data["initial_start"]["time"])
    itinerary.append(f"You start at {data['initial_start']['location']} at {format_time(current_time)}.")
    
    for meeting in data["meetings"]:
        travel_duration = timedelta(minutes=meeting["travel_duration"])
        current_time += travel_duration
        itinerary.append(f"You travel to {meeting['location']} in {meeting['travel_duration']} minutes and arrive at {format_time(current_time)}.")
        
        if meeting["waiting_time"] > 0:
            wait_until = parse_time(meeting["start_time"])
            itinerary.append(f"You wait until {format_time(wait_until)}.")
            current_time = wait_until
        
        meeting_start = parse_time(meeting["start_time"])
        meeting_end = parse_time(meeting["end_time"])
        meeting_duration = int((meeting_end - meeting_start).total_seconds() / 60)
        itinerary.append(f"You meet {meeting['person']} for {meeting_duration} minutes from {format_time(meeting_start)} to {format_time(meeting_end)}.")
        
        current_time = meeting_end
    
    return " ".join(itinerary)
<end_of_code>
\end{tcblisting}

\clearpage

\subsection{Output of Agents for Travel Planner}
\begin{tcblisting}{title=Output of Solution Agent, listing only, breakable}
<start_of_structured_output>
{
    "solutions": [
        {
            "day": 1,
            "current_city": "from Indianapolis to Grand Junction",
            "transportation": "Self-driving, from Indianapolis to Grand Junction",
            "breakfast": "-",
            "attraction": "-",
            "lunch": "-",
            "dinner": "-",
            "accommodation": "NYC Apartment near Central Park!, Grand Junction"
        },
        {
            "day": 2,
            "current_city": "Grand Junction",
            "transportation": "-",
            "breakfast": "Austin's BBQ and Oyster Bar, Grand Junction",
            "attraction": "Museum of the West, Museums of Western Colorado, Grand Junction",
            "lunch": "Punjab Da Pind, Grand Junction",
            "dinner": "Cha Bar, Grand Junction",
            "accommodation": "NYC Apartment near Central Park!, Grand Junction"
        },
        {
            "day": 3,
            "current_city": "from Grand Junction to Alamosa",
            "transportation": "Self-driving, from Grand Junction to Alamosa",
            "breakfast": "-",
            "attraction": "-",
            "lunch": "-",
            "dinner": "-",
            "accommodation": "Private & Quaint West Village Gem!, Alamosa"
        },
        {
            "day": 4,
            "current_city": "Alamosa",
            "transportation": "-",
            "breakfast": "Good Luck Cafe, Alamosa",
            "attraction": "San Luis Valley Museum | Alamosa, Alamosa",
            "lunch": "Lights Camera Action - Air Bar, Alamosa",
            "dinner": "Street Foods by Punjab Grill, Alamosa",
            "accommodation": "Private & Quaint West Village Gem!, Alamosa"
        },
        {
            "day": 5,
            "current_city": "from Alamosa to Denver",
            "transportation": "Self-driving, from Alamosa to Denver",
            "breakfast": "-",
            "attraction": "-",
            "lunch": "-",
            "dinner": "-",
            "accommodation": "GORGEOUS Newly-Renovated 2-BR Flat, Denver"
        },
        {
            "day": 6,
            "current_city": "Denver",
            "transportation": "-",
            "breakfast": "The Urban Socialite, Denver",
            "attraction": "Denver Zoo, Denver",
            "lunch": "Woods Spice, Denver",
            "dinner": "Radhika Sweets, Denver",
            "accommodation": "GORGEOUS Newly-Renovated 2-BR Flat, Denver"
        },
        {
            "day": 7,
            "current_city": "from Denver to Indianapolis",
            "transportation": "Self-driving, from Denver to Indianapolis",
            "breakfast": "-",
            "attraction": "-",
            "lunch": "-",
            "dinner": "-",
            "accommodation": "-"
        }
    ],
    "solutions_description": "The 'solutions' key contains a list of daily itineraries for a trip. Each day is represented as an object with the following keys: 'day' indicates the day number; 'current_city' shows the city or route for the day; 'transportation' describes the mode of transport and route; 'breakfast', 'lunch', and 'dinner' specify the meal locations and city; 'attraction' lists the places to visit; 'accommodation' provides the lodging details for the night. A '-' indicates no specific plan for that item."
}
<end_of_structured_output>
\end{tcblisting}


\begin{tcblisting}{title=Output of Planner Agent, listing only, breakable}
<start_of_COT>
Informations that are essential for generating combinations and filtering items :
- Each city requires an accommodation, an attraction, and 3 restaurants.
- Travel occurs on odd-numbered days, and staying in the same city occurs on even-numbered days.
- The last day involves traveling back to the starting location.
- Accommodations must be the same for two consecutive days in the same city.

Constraints that are essential for filtering plans :
- Accommodations must be "Entire home/apt" and have a maximum occupancy of 2.
- Transportation must not include flights.
- Restaurants must include Chinese, French, American, and Indian cuisines.
- The total budget for the trip is $3,800.
<end_of_COT>

<start_of_structured_output>
{
    "combinations": {
        "accommodations": {
            "Buffalo": 1,
            "Niagara Falls": 1,
            "New York": 1
        },
        "attractions": {
            "Buffalo": 1,
            "Niagara Falls": 1,
            "New York": 1
        },
        "restaurants": {
            "Buffalo": 3,
            "Niagara Falls": 3,
            "New York": 3
        },
        "transport": {
            "Greensboro_Buffalo": 1,
            "Buffalo_Niagara Falls": 1,
            "Niagara Falls_New York": 1,
            "New York_Greensboro": 1
        }
    },
    "constraints": {
        "restaurants": {
            "Cuisines": ["Chinese", "French", "American", "Indian"],
            "set_cover": []
        },
        "accommodations": {
            "room type": ["Entire home/apt"],
            "house_rules": [],
            "maximum occupancy": 2,
            "minimum nights": 2,
            "set_cover": []
        },
        "transport": {
            "mode": ["NOT flight"],
            "set_cover": []
        },
        "other_constraints": {
            "budget": 3800
        }
    },
    "combinations_description": "The 'combinations' key specifies the number of accommodations, attractions, restaurants, and transport options needed for each city. Each city requires one accommodation, one attraction, and three restaurants. Transport is needed for each leg of the journey between cities.",
    "constraints_description": "The 'constraints' key specifies the requirements for restaurants, accommodations, and transport. Restaurants must offer specific cuisines. Accommodations must be entire homes/apartments with a maximum occupancy of 2. Transport must not include flights. The budget constraint is $3,800."
}
<end_of_structured_output>

<start_of_planning>
{
    "Input Agent": "Identify the set of elements to generate permutations/combinations by extracting the cities to visit, the number of days, and the travel rules. Identify constraints by extracting preferences for accommodations, transport modes, restaurant cuisines, and budget from the query.",
    "Combination Function Generator Agent": "Create a function combinations_func() that generates possible plans by creating combinations of accommodations, attractions, and restaurants for each city, and transport options for each leg of the journey. Ensure the plans adhere to the travel rules provided.",
    "Solution Function Generator Agent": "Create a function plan_func() that filters the plans generated by combinations_func() using the constraints. Ensure that accommodations meet the room type and occupancy requirements, transport does not include flights, restaurants cover the specified cuisines, and the total cost does not exceed the budget. Return the plan that satisfies all constraints."
}
<end_of_planning>
\end{tcblisting}

\begin{tcblisting}{title=Output of Combination Function Generator Agent, listing only, breakable}
<start_of_COT>
To solve this problem, we need to generate travel plans based on the given parameters and reference data. The task involves creating a structured itinerary for a trip that includes accommodations, attractions, restaurants, and transportation between cities. Here's the step-by-step thought process:

1. **Identify Travel Order:**
   - Use the "transport" keys to determine the travel order. The starting city is identified by finding the city that is not a destination in any of the transport keys.
   - Follow the transport keys to determine the sequence of cities visited.

2. **Iterate Over Reference Data:**
   - The reference data is a list of elements, each representing a complete set of data for a trip. We need to iterate over each element to generate a plan.

3. **Generate Plans:**
   - For each element in the reference data, create a plan that spans multiple days.
   - On odd-numbered days, the traveler moves from one city to another. This requires transportation and accommodation.
   - On even-numbered days, the traveler stays in a city. This requires accommodation, breakfast, lunch, dinner, and an attraction.

4. **Structure of Each Day:**
   - **Odd Days (Travel Days):**
     - Transportation: Use the transport data for the current leg of the journey.
     - Accommodation: Use the accommodation data for the destination city.
     - Meals and Attraction: Set to "-".

   - **Even Days (Stay Days):**
     - Accommodation: Use the accommodation data for the current city.
     - Breakfast, Lunch, Dinner: Use the restaurant data for the current city.
     - Attraction: Use the attraction data for the current city.
     - Transportation: Set to "-".

5. **Return to Starting Location:**
   - On the last day, the traveler returns to the starting location. This requires transportation but no accommodation or meals.

6. **Output Format:**
   - Each plan is a list of dictionaries, where each dictionary represents a day in the itinerary.
   - Ensure the plans are structured according to the example provided.

By following these steps, we can systematically convert each element of the reference data into a structured travel plan.

<end_of_COT>

<start_of_code>
def combinations_func(parameters, reference_data):
    plans = []
    
    for data in reference_data:
        plan = []
        transport_keys = list(data['transport'].keys())
        
        # Determine the starting city
        cities = list(data['attractions'].keys())
        starting_city = None
        for key in transport_keys:
            from_city, to_city = key.split('_')
            if from_city not in cities:
                starting_city = from_city
                break
        
        # Determine the travel order
        travel_order = [starting_city]
        current_city = starting_city
        while len(travel_order) < len(cities) + 1:
            for key in transport_keys:
                from_city, to_city = key.split('_')
                if from_city == current_city:
                    travel_order.append(to_city)
                    current_city = to_city
                    break

        
        # Generate the plan
        day = 1
        for i in range(len(travel_order) - 1):
            from_city = travel_order[i]
            to_city = travel_order[i + 1]
            
            # Odd day: travel day
            plan.append({
                "day": day,
                "current_city": f"from {from_city} to {to_city}",
                "transportation": f"{data['transport'][f'{from_city}_{to_city}'][0]['name']}, from {from_city} to {to_city}",
                "breakfast": "-",
                "attraction": "-",
                "lunch": "-",
                "dinner": "-",
                "accommodation": f"{data['accommodations'][to_city][0]['name']}, {to_city}"
            })
            day += 1
            
            # Even day: stay day
            plan.append({
                "day": day,
                "current_city": to_city,
                "transportation": "-",
                "breakfast": f"{data['restaurants'][to_city][0]['name']}, {to_city}",
                "attraction": f"{data['attractions'][to_city][0]['name']}, {to_city}",
                "lunch": f"{data['restaurants'][to_city][1]['name']}, {to_city}",
                "dinner": f"{data['restaurants'][to_city][2]['name']}, {to_city}",
                "accommodation": f"{data['accommodations'][to_city][0]['name']}, {to_city}"
            })
            day += 1
        
        # Last day: return to starting location
        last_city = travel_order[-1]
        plan.append({
            "day": day,
            "current_city": f"from {last_city} to {starting_city}",
            "transportation": f"{data['transport'][f'{last_city}_{starting_city}'][0]['name']}, from {last_city} to {starting_city}",
            "breakfast": "-",
            "attraction": "-",
            "lunch": "-",
            "dinner": "-",
            "accommodation": "-"
        })
        
        plans.append(plan)
    
    return plans
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Solution Function Generator Agent, listing only, breakable}
<start_of_COT>
To solve the problem, we need to evaluate each plan against the given constraints and reference data. The constraints include budget, accommodation requirements, and transportation rules. We will follow these steps:

1. **Initialize Variables**: Set up necessary variables to track costs and transportation modes.

2. **Iterate Through Plans**: For each plan, check the following:
   - **Transportation**: Extract the mode and route. Ensure no conflicting modes (e.g., self-driving with flight or taxi). Calculate transportation costs based on the number of people and vehicle capacity.
   - **Accommodations**: Verify the minimum nights and calculate the cost based on occupancy.
   - **Restaurants**: Ensure no repeated restaurants and calculate meal costs.
   - **Budget**: Sum up all costs and check against the budget constraint.

3. **Check Constraints**: Ensure all constraints are satisfied, including transportation rules and budget.

4. **Select Valid Plan**: If a plan meets all constraints, return it. If no plan is valid, return the first plan.

5. **Error Handling**: Assume reference data is correct and handle any extraction errors by reporting them.

The function will return the first valid plan or the first plan if none are valid.
<end_of_COT>

<start_of_code>
import math

def plan_func(data, reference_data, constraints):
    num_people = constraints['accommodations']['maximum occupancy']
    budget = constraints['other_constraints']['budget']
    
    for plan in data:
        total_cost = 0
        transportation_set = set()
        visited_restaurants = set()
        valid_plan = True
        
        for day in plan:
            # Check transportation
            if day['transportation'] != "-":
                transport_name, from_to = day['transportation'].rsplit(',', 1)
                from_to = from_to.strip().replace("from ", "").replace(" to ", "_")
                
                transport_info = next((t for t in reference_data['transport'] if t['name'] == transport_name and t['from_to'] == from_to), None)
                if not transport_info:
                    raise ValueError("Transportation reference data not found.")
                
                transportation_set.add(transport_info['mode'])
                
                if transport_info['mode'] == 'self-driving':
                    transportation_cost = math.ceil(num_people / 5) * transport_info['cost']
                elif transport_info['mode'] == 'taxi':
                    transportation_cost = math.ceil(num_people / 4) * transport_info['cost']
                else:  # flight
                    transportation_cost = num_people * transport_info['cost']
                
                total_cost += transportation_cost
            
            # Check accommodation
            if day['accommodation'] != "-":
                accommodation_name, city = day['accommodation'].rsplit(',', 1)
                accommodation_info = next((a for a in reference_data['accommodations'] if a['name'] == accommodation_name and a['City'] == city.strip()), None)
                if not accommodation_info:
                    raise ValueError("Accommodation reference data not found.")
                
                if accommodation_info['minimum nights'] > constraints['accommodations']['minimum nights']:
                    valid_plan = False
                    break
                
                accommodation_cost = math.ceil(num_people / accommodation_info['maximum occupancy']) * accommodation_info['price_per_room']
                total_cost += accommodation_cost
            
            # Check restaurants
            for meal in ['breakfast', 'lunch', 'dinner']:
                if day[meal] != "-":
                    restaurant_name, city = day[meal].rsplit(',', 1)
                    if restaurant_name in visited_restaurants:
                        valid_plan = False
                        break
                    visited_restaurants.add(restaurant_name)
                    
                    restaurant_info = next((r for r in reference_data['restaurants'] if r['name'] == restaurant_name and r['City'] == city.strip()), None)
                    if not restaurant_info:
                        raise ValueError("Restaurant reference data not found.")
                    
                    meal_cost = num_people * restaurant_info['Average Cost Per Person']
                    total_cost += meal_cost
            
            if not valid_plan:
                break
        
        # Check transportation rules
        if ('self-driving' in transportation_set and 'flight' in transportation_set) or ('self-driving' in transportation_set and 'taxi' in transportation_set):
            valid_plan = False
        
        # Check budget
        if total_cost > budget:
            valid_plan = False
        
        if valid_plan:
            return plan
    
    return data[0]
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Output of Deliverer Function Generator Agent, listing only, breakable}
<start_of_COT>
1. The few-shot example solution is structured with a heading for each day, formatted as "Day X:", where X is the day number. Each day's details are listed under this heading, with each category (Current City, Transportation, Breakfast, Attraction, Lunch, Dinner, Accommodation) on a new line. The format is consistent, with each category followed by a colon and the corresponding information. If a category has no specific plan, it is represented by a "-".

2. To design the function, I will iterate over each day's itinerary in the input JSON. For each day, I will extract the relevant details and format them according to the pattern observed in the few-shot example. I will ensure that each day's details are prefixed with "Day X:" and that each category is followed by a colon and the corresponding information. If a category is "-", it will be displayed as such. The function will return a string that concatenates all the formatted day details.
<end_of_COT>

<start_of_code>
def deliver_func(data):
    result = []
    for day_plan in data:
        day_details = [
            f"Day {day_plan['day']}:",
            f"Current City: {day_plan['current_city']}",
            f"Transportation: {day_plan['transportation']}",
            f"Breakfast: {day_plan['breakfast']}",
            f"Attraction: {day_plan['attraction']}",
            f"Lunch: {day_plan['lunch']}",
            f"Dinner: {day_plan['dinner']}",
            f"Accommodation: {day_plan['accommodation']}"
        ]
        result.append("\n".join(day_details))
    return "\n\n".join(result)
<end_of_code>
\end{tcblisting}

==> Sections/prompts_full.tex <==
\subsection{Prompts for Agents for Natural Plan}
\needspace{6\baselineskip}

\begin{tcblisting}{title=Prompt for Solution Agent, listing only, breakable}
You are a Solution Agent. 

You are given a solution. Based on the solution, you have to create a structured output for the solution in list or JSON.
You are also required to provide the description of keys and values of the solution.
Please use as less keys as possible to represent the solution in structured output. For example in trip planning, the name of cities and list of visiting days are enough to provide the solution, hence only two keys are required. 

Your output format is as below:

<start_of_structured_output>
{
    "solutions": <The solutions>,
    "solutions_description": <Field description of 'solutions' key. Please describe the keys and values in detail>
}
<end_of_structured_output>

For number-based values, please do not use string. If the value is range based, please use list instead.
Please ensure your JSON is in correct format and able to be parsed. Please do not write the field description for "solutions_description" in dictionary, only string is allowed.


Solution:
<few_shot_examples_solution>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Planning Agent, listing only, breakable}
You are a combinations and constraints planning agent. 

You are given few-shot examples queries and structured solution corresponding to the query. Based on the few-shot examples, you have to define them as general constraints planning problems. You identify the ways to generate possible combinations of plans and how to filter those plans to retrieve the solution.
You have three agents to assist you in solving the problem. The three agents are :

1. Input Agent - The agent provides set of elements to generate permutations/combinations and constraints as a structured JSON.
2. Combination Function Generator Agent - The agent creates a generic function called combinations_func() that takes any set of elements provided by Input Agent to generate the list of possible plans.
3. Filter Function Generator Agent - The agent creates a generic function called plan_func() that takes in the constraints provided by Input Agent and any list of possible plans outputted by the function created by Combination Function Generator Agent, to generate the most optimal plan that meets the constraints.

Based on the few-shot examples queries, you should observe what is considered valid possible combinations, and instruct Combination Function Generator Agent to produce those valid possible combinations.
You should identify whether the query is a constraints satisfaction problem (CSP) or optimisation problem. If it is a CSP problem, you should instruct the Filter Function Generator Agent to return the plan if it satisfied all constraints, else if it is an optimisation problem, you should instruct Filter Function Generator Agent to go through all plans that satisfied the constraints return the best one. You can only instruct the agent to either return any valid plan or return the best plan, not both.

Based on the few-shot examples queries, you convert the combination parameters and constraints in few-shot examples into structured output in JSON.
The keys should be "combinations" and "constraints" and respectively.

Then, based on the strucuted output you wrote, your instructions to each agent should cover the following:
1. Input Agent - You instruct the agent on how to identify the set of elements to generate permutations/combinations given a query. You also instruct the agent on how to identify the constraints to tackle such problems. The output format should consist of three keys: "combinations", "constraints" and "solutions", similar to the structured output that you wrote.
2. Combination Function Generator Agent - The "combinations" from the output of Input Agent will be the combinations_func() input. Hence, based on the output format of "combinations", you instruct the agent on creating a function on how to use the keys to generate possible plans.  The function is expected to output list of plans with each plan's format is similar to the few-shot structured solution. This output will be given to plan_func().
3. Filter Function Generator Agent - The "constraints" from the output of Input Agent and output of combinations_func() will be the plan_func() input. Based on the output format of "constraints" and "plan", as well as the type of problem, you instruct the agent on creating a function on how to use the keys from "constraints" to filter the plans from "plan". The function is expected to output a plan that matches the format of few-shot structured solution.

Before providing the structured output, you must output Chain-of-Thought (CoT):
1. First, you must analyse the few-shot examples structured solution. For each key in the solution, you must mention what information are essential in point form. All of the information that you listed must be given to "combinations" in your structured output to generate plans that obey the format of structured solution.
2. Then, you must analyse what are the information that could help filter out all the combination of plans. These information are essential to be given to "constraints" to obtain plan that meet the constraints.

Please do not write the instructions in dictionary, only string is allowed. Please ensure time is in HH:MM format.

Your output format is as below:

<start_of_COT>
Informations that are essential for generating combinations :
<informations in point form>

Constraints that are essential for filtering plans :
<informations in point form>
<end_of_COT>

<start_of_structured_output>
{
    "combinations": <The set of parameters that generate permutations/combinations>,
    "constraints": <The set of constraints>,
    "combinations_description": <Field description of the value in 'combinations' key. Please describe the keys and values in detail. Please ensure it is written in string and not dict.>,
    "constraints_description": <Field description of 'constraints' key. Please describe the keys and values in detail. Please ensure it is written in string and not dict.>,
}
<end_of_structured_output>

<start_of_planning>
{
    "Input Agent": <Your instructions for Input Agent>,
    "Combination Function Generator Agent": <Your instructions for Combination Function Generator Agent>,
    "Filter Function Generator Agent": <Your instructions for Solutions Function Generator Agent>
}
<end_of_planning>

All of your instructions must be as general as possible. For example, you should not mention any specific cities, days or flights, so that the instructions can be applied to other queries than the queries provided to you.
Please ensure your JSON is in correct format and able to be parsed. Do not use "..." to indicate more items.

Few-Shot Examples Query:
<few_shot_examples_query>

Few-Shot Examples Structured Solution:
<few_shot_examples_solution>

Few-Shot Examples Structured Solution Description:
<few_shot_examples_solution_description>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Combination Function Generator Agent, listing only, breakable}
You are the Combination Function Generator Agent. 

You are given such instructions:
<instructions>

You have to follow the provided instructions to create a function that generate a list of possible combinations of plans. The input parameter of the function 'data', which is a dictionary. You should refer to the provided description of input format, example of input, output format and example of output to design your function.

The description of input format is follows:
<input_description>

An example of input is as follows:
<example_input>

The description of output format for each plan is as follows:
<output_description>

An example of a plan is as follows:
<example_output>

Please use product in Python library itertools to help you in your code. Don't use other libraries like cycle (You don't need them). Please do not use recursive function as it will make the code complicated.

The name of the function you will generate is "combinations_func()". Please do not include any example usage or print anything in your code.


WARNING: Only apply instructions that are explicitly stated. Do not assume fairness, balance, or symmetry unless specified. Your function must return a list, not a dict.

Before you write your function code, you must output Chain-of-thought (CoT), which you explain your thought-process and programming logic in order to match the output format provided to you.


Do not ever hardcode any information. If such information is not provided, please do not use it.

Your output format is as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your combinations_func() code>
<end_of_code>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Combination Function Reflection Agent, listing only, breakable}
You are a Reflection Agent. Your job is to observe the mistake of the output of the Combination Function Generator Agent.

The job of Combination Function Generator Agent is to create a function called combinations_func() that generate a list of possible combinations of plans. The input parameter of the function 'data', which is a dictionary.
However, the agent made a mistake in the function that causes the function to not able to generate combinations of plans that contain the ground-truth plan.

Here is the one of the output plan from the list of plans provided by the function:
<example_input>

Here is the expected ground-truth plan that the generated combinations of plans should contain:
<example_output>

Here is the Chain-of-Thought (CoT) thought process of the agent before writing the code:
<chain_of_thought>

Here is the code written by the agent:
<code>

Your main job is as follows: 
1. You observe the pattern of ground-truth plan and the pattern of one of the output plan from the list of plans. You mention the difference in pattern in your CoT.
2. You should also mention in your CoT that how you should change the CoT thought process of agent to ensure the function generates plan with consistent pattern as the ground-truth plan. 
3. You correct the CoT of the agent and write it in your output. Then, you made the corresponding correction on the agent's code.
4. Please do not hardcode the function to append the ground-truth plan to the solution. Please do not check the combinations against the ground-truth plan. This defeat the purpose of ensuring the function generates valid plans. Similarly like the original code, the final function should output a list, not a dict. Do not use wrapper like ```python``` when writing code. Use the wrapper in the provided output format.


Your output format is as follows:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_COT_correction>
<corrected CoT of Combination Function Generator Agent>
<end_of_COT_correction>

<start_of_code_correction>
<corrected code of Combination Function Generator Agent>
<end_of_code_correction>


\end{tcblisting}

\begin{tcblisting}{title=Prompt for Filter Function Generator Agent, listing only, breakable}
You are the Filter Function Generator Agent. 

You are given such instructions:
<instructions>

You have to follow the provided instructions to create a function that retrieve the desired plan. The input parameter of the function are 'data' and 'constraints'. 'Data' contains a list of plan, with each plan in JSON format. 'Constraints' contains the constraints. You should refer to the provided description of input plan format, example of input, description of constraints format and example of constraints to design your function.
Your function will return one of the plans as solution.

You are given a list of plan, the description of input format for each plan is as follows:
<input_description>

An example of a plan is as follows:
<example_input>

You are also given the constraints, the description of constraints for is as follows:
<constraints_description>

An example of constraints is as follows:
<example_constraints>

The name of the function you will generate is "plan_func()". Please do not include any example usage or print anything in your code.

Remember, the input parameter "data" is a list, while the input parameter "constraints" is JSON.

Your output is a Chain-of-thought (CoT) and Python function as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your plan_func() code>
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Filter Function Reflection Agent, listing only, breakable}
You are a Reflection Agent. Your job is to observe the mistake of the output of the Filter Function Generator Agent.

The job of Filter Function Generator Agent is to create a function called plan_func() that returns the valid plan given a list of possible combinations of plans. The input parameter of the function are 'data' and 'constraints'. 'Data' contains a list of plan, with each plan in JSON format. 'Constraints' contains the constraints. You should refer to the provided description of input plan format, example of input, description of constraints format and example of constraints to design your function.
However, the agent made a mistake in the function that causes the function to not able to return the ground-truth plan from the possible combinations of plans.

Here is the instructions given to the agent:
<instructions>

Here is the expected ground-truth plan that the function should return:
<example_output>

Here is the plan that the function returns:
<function_output>

Here is the Chain-of-Thought (CoT) thought process of the agent before writing the code:
<chain_of_thought>

Here is the code written by the agent:
<code>

Your main job is as follows: 
1. You observe the difference between ground-truth plan and the plan that the function returns.
2. If the function returns None, it indicates a constraint is handled incorrectly in the code that some plans might meet it but overlooked by the function. Check whether is there possibility that each constraint can be handled differently that some plans can meet such constraints. 
3. If the function does not return None but returns a different plan than ground-truth, you should reflect whether some constraints are written too lenient that some plans might not meet the constraints but overlooked by the function.
4. Once you identified the constraint that is handled incorrectly, you should mention in your CoT that how you should change the CoT thought process of agent to ensure the function handles the constraints correctly. 
5. You correct the CoT of the agent and write it in your output. Then, you made the corresponding correction on the agent's code. 
6. Please do not hardcode the function to return the ground-truth plan to the solution. This defeat the purpose of ensuring the function returns the correct plan. Similarly like the original code, the final function should output a JSON. Do not use wrapper like ```python``` when writing code. Use the wrapper in the provided output format.


Your output format is as follows:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_COT_correction>
<corrected CoT of Filter Function Generator Agent>
<end_of_COT_correction>

<start_of_code_correction>
<corrected code of Filter Function Generator Agent>
<end_of_code_correction>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Deliverer Function Generator Agent, listing only, breakable}
You are the Deliverer Function Generator Agent. 

Given an input, you have to create a function that processes the input and provides output that matches the format of few-shot examples solution. The input parameter of the function 'data', which is a plan in JSON. You should refer to the provided description of input plan format and example of input to design your function.

You are given a plan, the description of a plan is as follows:
<input_description>

An example of a plan is as follows:
<example_input>

The few-shot example solution is as follows:
<few_shot_examples_solution>

The name of the function you will generate is "deliver_func()". Please do not include any example usage or print anything in your code.

Before writing your code, you must output Chain-of-thought (CoT):
1. You must first analyse the format of few-shot example solution. Does it contain any heading? What does the pattern of output look like?
2. Then, you explain how are you going to design the function to ensure the format of your function's output is consistent with the few-shot example solution. Do not miss any heading if the example solution contains heading.

Your output format is CoT and Python function as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your deliver_func() code>
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Deliverer Function Reflection Agent, listing only, breakable}
You are a Reflection Agent. Your job is to observe the mistake of the output of the Deliverer Function Generator Agent 

The job of Deliverer Function Generator Agent us to create a function that processes a structured input in JSON and provides output that matches the format of few-shot examples solution in natural language. The input parameter of the function 'data', which is a plan in JSON.
However, the agent made a mistake in designing the function, resulting in the output of function does not match the format of few-shot examples solution in natural language, despite the structured input is correct.
The name of the function you will generate is "deliver_func()". The input parameter of function is "data", which is structured input.

Here is the structured input given to the function:
<structured_input>

Here is the expected ground-truth plan from the few-shot examples:
<example_output>

Here is the plan that the function returns:
<current_output>

Here is the code written by the agent:
<code>

Your main job is as follows: 
1. You observe the pattern of ground-truth plan and the pattern of plan that the function returns. You mention the difference in pattern in your CoT.
2. You should also mention in your CoT that how you should change the code to ensure the function generates plan with consistent pattern as the ground-truth plan. 
3. You correct the CoT of the agent and write it in your output. Then, you made the corresponding correction on the agent's code.
4. Please do not hardcode the function to return the ground-truth plan from few-shot examples. Please do not check the output of function against ground-truth plan from few-shot examples. This defeat the purpose of ensuring the function generates plans with valid format. Similarly like the original code, the final function should be a string. Do not use wrapper like ```python``` when writing code. Use the wrapper in the provided output format.

You must ensure the format of your function's output is consistent with the example solution. Do not miss any header if the example solution contains header.

Your output is a Chain-of-thought (CoT) and Python function as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your deliver_func() code>
<end_of_code>
\end{tcblisting}

\begin{tcblisting}{title=Prompt for Input Agent, listing only, breakable}
You are the Input Agent. 

You are given such instructions:
<instructions>

The description of output format is as follows:
<output_description>

An example of query is given below:
<example_input>

An example of output is given below:
<example_output>

You will be given a query. You have to generate a strcutured output in JSON adhering to the provided instructions and output format. You should refer to the provided description of output format and example of output. 


Your output format is as below:
<start_of_structured_output>
<your structured output>
<end_of_structured_output>

Query :
<query>

\end{tcblisting}

\clearpage

\subsection{Prompts for Agents for Travel Planner}

\needspace{6\baselineskip}

\begin{tcblisting}{title=Prompt for Solution Agent, listing only, breakable}
You are a Solution Agent. 

You are given a solution. Based on the solution, you have to create a structured output for the solution in list or JSON.
You are also required to provide the description of keys and values of the solution.
Please use as less keys as possible to represent the solution in structured output. For example in trip planning, the name of cities and list of visiting days are enough to provide the solution, hence only two keys are required. 

Your output format is as below:

<start_of_structured_output>
{
    "solutions": <The solutions>,
    "solutions_description": <Field description of 'solutions' key. Please describe the keys and values in detail>
}
<end_of_structured_output>

For number-based values, please do not use string. If the value is range based, please use list instead.
Please ensure your JSON is in correct format and able to be parsed. Please do not write the field description for "solutions_description" in dictionary, only string is allowed.


Solution:
<few_shot_examples_solution>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Planning Agent, listing only, breakable}
You are a combinations and constraints planning agent. 

You are given few-shot examples queries and structured solution corresponding to the query. Based on the few-shot examples, you have to define them as general constraints planning problems. You identify the ways to generate possible combinations of plans and how to filter those plans to retrieve the solution.
You have three agents to assist you in solving the problem. The three agents are :

1. Input Agent - The agent provides set of elements to generate permutations/combinations and constraints as a structured JSON.
2. Combination Function Generator Agent - The agent creates a generic function called combinations_func() that takes any set of elements provided by Input Agent to generate the list of possible plans.
3. Filter Function Generator Agent - The agent creates a generic function called plan_func() that takes in the constraints provided by Input Agent and any list of possible plans outputted by the function created by Combination Function Generator Agent, to generate the most optimal plan that meets the constraints.

Based on the few-shot examples queries, you should observe what is considered valid possible combinations, and instruct Combination Function Generator Agent to produce those valid possible combinations.
You should identify whether the query is a constraints satisfaction problem (CSP) or optimisation problem. If it is a CSP problem, you should instruct the Filter Function Generator Agent to return the plan if it satisfied all constraints, else if it is an optimisation problem, you should instruct Filter Function Generator Agent to go through all plans that satisfied the constraints return the best one. You can only instruct the agent to either return any valid plan or return the best plan, not both.

Based on the few-shot examples queries, you convert the combination parameters and constraints in few-shot examples into structured output in JSON.

You are given few shot examples options for the items. Your combination parameters should only provide values based on the few-shot options.
You also need to mention which combination parameters are set covers, which means that each item in the data potentially only cover a part of the parameter value, and require multiple data to together cover all the values in the parameter.

The keys should be "combinations" and "constraints" and respectively.

Then, based on the strucuted output you wrote, your instructions to each agent should cover the following:
1. Input Agent - You instruct the agent on how to identify the set of elements to generate permutations/combinations given a query. You also instruct the agent on how to identify the constraints to tackle such problems. The output format should consist of three keys: "combinations", "constraints" and "solutions", similar to the structured output that you wrote.
2. Combination Function Generator Agent - The "combinations" from the output of Input Agent will be the combinations_func() input. Hence, based on the output format of "combinations", you instruct the agent on creating a function on how to use the keys to generate possible plans. The function is expected to output list of plans with each plan's format is similar to the few-shot structured solution. This output will be given to plan_func().
3. Filter Function Generator Agent - The "constraints" from the output of Input Agent and output of combinations_func() will be the plan_func() input. Based on the output format of "constraints" and "plan", as well as the type of problem, you instruct the agent on creating a function on how to use the keys from "constraints" to filter the plans from "plan". The function is expected to output a plan that matches the format of few-shot structured solution.

Before providing the structured output, you must output Chain-of-Thought (CoT):
1. First, you must analyse the few-shot examples structured solution and rule of generating combination of plan. Then, you must mention the number of each key required for the whole plan.
2. Please DO NOT include any information in the options in the "combinations".
2. Then, you must analyse what are the information in the options could help filter out items using the options. These information are essential to be given to "constraints" to obtain item that meet the constraints.
3. Finally, you must analyse what are the information NOT in the options could help filter out the plans that do not meet such constraints. These information are essential to be given to "constraints" to obtain plan that meet the constraints. 

The rule of generating combination of plan is as follows :
1. Travel to another location in odd number day and staying in the same city at even number.
2. When staying in each city, an accommodation, an attractions and 3 restaurants are required. You are required to stay in the same accommodation in the city for two days. 
3. For the last day, you are required to travel back to the starting location.
4. You don't have to add these rules as constraints in your structured output.

For your structured output, you must fill in the values specific to the query.

Please do not write the instructions in dictionary, only string is allowed.

Your output format is as below:

<start_of_COT>
Informations that are essential for generating combinations and filtering items :
<informations in point form>

Constraints that are essential for filtering plans :
<informations in point form>
<end_of_COT>

<start_of_structured_output>
{
    "combinations": <combinations_format>,
    "constraints": <constraints_format>,
    "combinations_description": <Field description of the value in 'combinations' key. Please describe the keys and values in detail>,
    "constraints_description": <Field description of 'constraints' key. Please describe the keys and values in detail>,
}
<end_of_structured_output>

<start_of_planning>
{
    "Input Agent": <Your instructions for Input Agent>,
    "Combination Function Generator Agent": <Your instructions for Combination Function Generator Agent>,
    "Filter Function Generator Agent": <Your instructions for Solutions Function Generator Agent>
}
<end_of_planning>

All of your instructions must be as general as possible. For example, you should not mention any specific cities, days or flights, so that the instructions can be applied to other queries than the queries provided to you.
Please ensure your JSON is in correct format and able to be parsed. Do not use "..." to indicate more items.

Few-Shot Examples Query:
<few_shot_examples_query>

Few-Shot Examples Structured Solution:
<few_shot_examples_solution>

Few-Shot Examples Structured Solution Description:
<few_shot_examples_solution_description>

Few-Shot Examples Options:
<few_shot_examples_options>

Few-Shot Examples Combinations Input:
<few_shot_examples_solution>


\end{tcblisting}

\begin{tcblisting}{title=Prompt for Combination Function Generator Agent, listing only, breakable}
You are the Combination Function Generator Agent. 

You are given such instructions:
<instructions>

You have to follow the provided instructions to convert the each element of reference data into plans. The input parameter of the function are 'parameters' and 'reference_data', both are dictionaries. You should refer to the provided example of parameters, element of reference data and example of output to design your function.

The description of parameters is follows:
<input_description>

An example of parameters is as follows:
<example_parameters>

An example of an element of reference data is as follows:
<example_reference_data>

An example of a plan is as follows:
<example_output>


The main function of your code is to convert the format from reference data to the format of plan. The reference data is a list of elements, which each element can be converted to a single plan.
Each element has contained sufficient information to produce a plan, you do not need to further generate combinations or permutations via itertools.
Hence, you need to iterate each element to convert them into each plan and store them in a list and return the list.

You must follow the pattern of example plan. Like travelling to another location in odd number day and staying in the same city at even number. When travelling or staying in, you must also see whether accommodation, attractions and restaurants are required. For the last day, you are required to travel back to the starting location.

The name of the function you will generate is "combinations_func()".
Before you write your function code, you must output Chain-of-thought (CoT), which you explain your thought-process and programming logic in order to match the output format provided to you.
Do not ever hardcode any information, for example total days. If such information is not provided, please do not use it.

The format of key in "transport" is {from}_{to}. There is only one travel city order from the "transport". You can easily figure out the travel order by the key in "transport".
You can determine the travel order as follows:
1. The keys from "attractions" shows the cities the user is going to visit, so you can figure out the "starting point" where the {from} in "transport" does not belong to the keys in "attractions".
2. The second location is going to be where the key exists in "transport": {starting_location}_{second_location}.
3. Use an iterative approach to find the travel order.

You are reminded that reference data is a list of elements that should be converted to a plan, not just a single element.
Please don't hardcode the transportation as there are more options than self-driving. The element of reference data will show what transport is needed to travel from one city to another.
Please make sure the plans are in odd number. User is travelling from one city to another in odd day and staying in a city in even day. In even day, restaurants and attractions are required. Every day except the last day, accommodation is required. At the last day, user travels back to starting location.
All information are provided in reference data. Remember, accommodation is needed on the first day.

Your output format is as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your combinations_func() code>
<end_of_code>

\end{tcblisting}

\begin{tcblisting}{title=Prompt for Filter Function Generator Agent, listing only, breakable}
You are the Filter Function Generator Agent. 

You have to follow the provided instructions to create a function that retrieve the desired plan. The input parameter of the function are 'data', 'reference_data' and 'constraints'. 'Data' contains a list of plans. 'Reference_data' contains the data you need to refer to when checking whether the plan meets constraints. 'Constraints' contains the constraints. You should refer to the example of input, description of constraints format and example of constraints to design your function.
Your function will return one of the plans as solution.

An example of a plan is as follows:
<example_input>

An example of constraints is as follows:
<example_constraints>

An example of reference data is as follows:
<example_reference_data>

The name of the function you will generate is "plan_func()". Please do not include any example usage or print anything in your code.
Remember, the input parameter "data" is a list, while the input parameter "constraints" is JSON.

The name of restaurants, accommodations and attractions in the plan are in such format : <name>, <city>
Please note that it is possible that commas exist in <name>, so you should separate from the last comma.
You should assume given the correct name and city, you will definitely extract that item from reference data, so please report error instead if you cannot extract the item.
You should assume if the accommodation room maximum capacity exceeds the number of people, the user will still consider staying in the accommodation. However, the user will book multiple rooms of the same accommodation. You may use math.ceil to help you.
However, if the accommodation room minimum nights exceed the query's minimum nights, the plan will fail.

The name of transporation in the plan are in such format : <name>, <from_to>
Please note that it is possible that commas exist in <name>, so you should separate from the last comma.
The <from_to> has to be further processed because the <from_to> that you extract are in such format "from <from_location> to <to_location>".
You should assume given the correct name and from_to, you will definitely extract that item from reference data, so please report error instead if you cannot extract the item.
If user is taking flight, the user should buy tickets for everyone in the trip. The cost for flight is per ticket. The "mode" for flight is "flight".
You should also assume a self-driving car can fit 5 people while a taxi car can fit 4 people. If the number of people in the trip exceeds the capacity of vehicle (for example taxi), you assume the user will book multiple vehicles (for example multiple taxis). You may use math.ceil to help you.

You need to consider costs from restaurants, accommodations and transporation when dealing with budget constraints.

Assume the variable "maximum occupancy" in constraints is number of people.
Your solution should not handle travel dates.

If no plan meets all the constraints, you should return the first plan in data. Your function must provide at least one plan.

Do not write function that only particularly handle the specific constraints from example. Instead, write a general function that can handle constraints of any values.

You are assumed to handle both of these rules as well:
1. You are not allowed to have 'self-driving and flight' or 'self-driving and taxi' in a trip. 
2. You are not allowed to have repeated restaurants throughout the trip. 


You don't have to handle any missing reference entry (e.g. not being able to look up an accommodation, restaurant or transportation route). You assume reference entry is always in correct format.
However, you must handle this constraint : You are not allowed to have 'self-driving and flight' or 'self-driving and taxi' in a trip. 
Use a dictionary to store the transportation types and check if self-driving and flight' or 'self-driving and taxi' exist. If yes, plan is invalid.
transportation_set = set(). If ('self-driving' in transportation_set and 'flight' in transportation_set) or ('self-driving' in transportation_set and 'taxi' in transportation_set), plan is invalid.
Also, please ensure self-driving car can fit 5 people while a taxi car can fit 4 people. If the number of people in the trip exceeds the capacity of vehicle (for example taxi), you assume the user will book multiple vehicles (for example multiple taxis). You may use math.ceil to help you.
If taxi, transportation_cost = math.ceil(num_people / 4) * taxi_cost. If self-driving, ransportation_cost = math.ceil(num_people / 4) * self-driving_cost.


Your output is a Chain-of-thought (CoT) and Python function as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your plan_func() code. Don't wrap your code with ```python```>
<end_of_code>


\end{tcblisting}

\begin{tcblisting}{title=Prompt for Deliverer Function Generator Agent, listing only, breakable}
You are the Deliverer Function Generator Agent. 

Given an input, you have to create a function that processes the input and provides output that matches the format of few-shot examples solution. The input parameter of the function 'data', which is a plan in JSON. You should refer to the provided description of input plan format and example of input to design your function.

You are given a plan, the description of a plan is as follows:
<input_description>

An example of a plan is as follows:
<example_input>

The few-shot example solution is as follows:
<few_shot_examples_solution>

The name of the function you will generate is "deliver_func()". Please do not include any example usage or print anything in your code.

Before writing your code, you must output Chain-of-thought (CoT):
1. You must first analyse the format of few-shot example solution. Does it contain any heading? What does the pattern of output look like?
2. Then, you explain how are you going to design the function to ensure the format of your function's output is consistent with the few-shot example solution. Do not miss any heading if the example solution contains heading.

Your output format is CoT and Python function as below:
<start_of_COT>
<your COT>
<end_of_COT>

<start_of_code>
<your deliver_func() code>
<end_of_code>


\end{tcblisting}

\begin{tcblisting}{title=Prompt for Input Agent, listing only, breakable}
You are the Input Agent. 

You are given such instructions:
<instructions>

An example of query is given below:
<example_input>

The options corresponding to the query is given below:
<example_options>

An example of output expected by Input Agent is given below:
<example_output>



You will be given a query and options corresponding to the query. You have to generate a structured output in JSON adhering to the provided instructions and output format. You should refer to the example output to understand the output format.
You will also be given the combinations format, for you to generate the "combinations" in your output.


Here are the rules to provide structured output :
1. Please DO NOT include any information in the options in the "combinations". In your "combinations" for each key, you should refer to "cities_to_visit" from options to fill in the exact name of city. Please do not hallucinate and provide cities that are not mentioned in the options.
2. Some of the key in the constraints have options. You can only use the input in the options (that will be provided to you) to fill in the values of the key of "constraints". If the query does not mention any constraint for that key, leave the list empty.
3. For options to be filtered instead of retain, add a 'NOT' before the options.

The rules of travelling is as follows :
1. Travel to another location in odd number day and staying in the same city at even number.
2. When staying in each city, an accommodation, an attractions and 3 restaurants are required. You are required to stay in the same accommodation in the city for two days. 
3. For the last day, you are required to travel back to the starting location.
4. If no number of people are mentioned in the query, you should assume only 1 person is travelling.
5. Please do not put empty list or [] as "maximum occupancy". It must be an integer. "maximum occupancy" must be an integer.
6. If the query mentions "group of N" people, you should assume N number of people travelling. "maximum occupancy" = N.

Your output format is as below:
<start_of_structured_output>
<your structured output>
<end_of_structured_output>

Query :
<query>

Options for constraints :
<options>

The format of combinations of your output is given below:
<combinations_format>
\end{tcblisting}


\clearpage

\subsection{Prompts for Planning Optimization Agent}

\needspace{6\baselineskip}

\begin{tcblisting}{title=Prompt for Removing Unnecessary Parameters, listing only, breakable}
You are a Planning Optimisation Agent. Your job is to filter out unnecessary parameters of the Planning Agent.

You will be given the output of Planning Agent. There are two outputs of Planning Agent:
1. Structured output - The agent will provide the combinations and constraints based on the few-shot examples, as well as their corresponding field description.
2. Planning instructions - The agent will write instructions to "Combination Function Generator Agent" and "Filter Function Generator Agent".

Here is the structured output of Planning Agent:
<structured_output>

Here is the planning instructions of Planning Agent:
<planning>

Your main job is as follows:
1. We define parameter as each key in the "combinations" and "constraints" from structured output. You are required to look at constraints that are not represented in list or JSON. You can assume constraints represented in list or JSON have discriminative power, as constraints represented in list or JSON have specific details to filter out some plans.
2. If the parameter has no discriminative power, the parameter has to be removed. We define the parameter with no discriminative power the constraint will either cause all plans to pass or fail. On the other hand, parameter that can cause one plan to fail and other plan to not fail have discriminative power.
3. For example, given the problems produces plan A, B and C, where sum of X for plan A, B and C have the same value, due to plan A,B and C have constant set of items, hence the parameter corresponding to the sum of X should be removed, because it will cause either all plans to pass or fail.
4. If the parameter should be removed, you should remove it in the structure output.
5. Hence, we define the parameter with no discriminative power based on two criteria : (i) The parameter applies uniformly across all of the plans. (ii) The parameter is not represented in list or JSON.

You MUST consider each key from BOTH "combinations" and "constraints" of the structured output as your parameters.
Please ensure your JSON is in correct format and able to be parsed. Do not use "..." to indicate more items.

Your output format is as follows:
<start_of_COT>
1. <Parameter Type 1> - <Justify whether the parameter applies/does not apply uniformly across all of the plans>. <Mention if the parameter is represented in list or JSON>. <Mention if the parameter has/does not have discriminative power>. Hence, it should be <removed/not removed>.
...
N. <Parameter Type N> - <Justify whether the parameter applies/does not apply uniformly across all of the plans. <Mention if the parameter is represented in list or JSON>. <Mention if the parameter has/does not have discriminative power>. Hence, it should be <removed/not removed>.
<end_of_COT>

<start_of_structured_output>
<Your structured output. The ignored parameters should be removed from the structured output>
<end_of_structured_output>

<start_of_planning>
<your planning>
<end_of_planning>


\end{tcblisting}




\begin{tcblisting}{title=Prompt for Moving Parameters to Combinations, listing only, breakable}
You are a Planning Optimisation Agent. Your job is to observe the validity of output of the Planning Agent.

You will be given the output of Planning Agent. There are two outputs of Planning Agent:
1. Structured output - The agent will provide the combinations and constraints based on the few-shot examples, as well as their corresponding field description.
2. Planning instructions - The agent will write instructions to "Combination Function Generator Agent" and "Filter Function Generator Agent".

Here is the structured output of Planning Agent:
<structured_output>

Here is the planning instructions of Planning Agent:
<planning>

Your main job is as follows:
1. You are only required to look at the constraints in the "constraints" of structured output, not "combinations".
2. Even if the constraint only applies to each item but not all items, you must also see if similar type of constraint applies to other items. You must properly check if the same type of constraints exists for every item in the combination space.
3. For example, given the combination space has item A, B and C, and the given type of constraint has 3 constraints, where each constraint is applied to A, B and C, then the same type of constraint exists for every item in the combination space.
4. If true, then that constraint is a combination parameter, which should be moved to "combinations" in structured output.

Please ensure your JSON is in correct format and able to be parsed. Do not use "..." to indicate more items.

Your output format is as follows:
<start_of_COT>
1. <Constraint Type 1> - <Justify whether the type of constraint exists/does not exist in every item in the combination space>. Hence, it is <combination parameters/constraint>.
...
N. <Constraint Type N> - <Justify whether the type of constraint exists/does not exist in every item in the combination space>. Hence, it is <combination parameters/constraint>.
<end_of_COT>

<start_of_structured_output>
<Your structured output. The constraints that are combination parameter should be moved to "combinations">
<end_of_structured_output>

<start_of_planning>
<your planning>
<end_of_planning>

\end{tcblisting}



\begin{tcblisting}{title=Prompt for Expanding Parameters Value, listing only, breakable}
You are a Planning Optimisation Agent. Your job is to observe the validity of output of the Planning Agent.

You will be given the output of Planning Agent. There are two outputs of Planning Agent:
1. Structured output - The agent will provide the combinations, constraints and structured solution based on the few-shot examples, as well as their corresponding field description.
2. Planning instructions - The agent will write instructions to "Combination Function Generator Agent" and "Filter Function Generator Agent".

Here is the list of type of constraints of Planning Agent:
<constraints>

Here is the structured output of Planning Agent:
<structured_output>

Here is the planning instructions of Planning Agent:
<planning>

Your main job is as follows:
1. We define parameter as each key in the "combinations" and "constraints" from structured output. For each type of parameter, you should check if the type of parameter is expandable. Check if there are any that suggest other parameters should also hold, even if they are not explicitly listed. Rewrite each type of parameters if you think it can be expanded.
2. For example, if pair [A,B] exists, then [B,A] might exist, despite not explicitly stated. Hence, such parameter can be expanded. You output Chain-of-Thought to explain your thought process of checking the claim of each parameter and explain whether the parameter is expandable.
3. You should assume the parameter can be expanded unless there are rules that explicitly stated such expansion cannot be done.

You MUST consider each key from BOTH "combinations" and "constraints" of the structured output as the parameter to analyse.
Please ensure your JSON is in correct format and able to be parsed. Do not use "..." to indicate more items.

Your output format is as follows:
<start_of_COT>
1. <Parameter Type 1> - <Justify whether the type of parameter is expandable>. Hence, it is <expandable/non-expandable>.
...
N. <Parameter Type N> - <Justify whether the type of parameter is expandable>. Hence, it is <expandable/non-expandablet>.
<end_of_COT>

<start_of_structured_output>
<Your structured output. For the type of parameter that it is expandable, you should write the expanded parameter>
<end_of_structured_output>

<start_of_planning>
<Please rewrite the planning instructions in JSON based on the format of the given planning instructions.>
<end_of_planning>
\end{tcblisting}



\begin{tcblisting}{title=Prompt for Filling Up Missing Parameters, listing only, breakable}
You are a Planning Optimisation Agent. Your job is to check if there are missing information in the structured output.

You will be given the output of Planning Agent. There are three outputs of Planning Agent:
1. Chain-of-Thought - The agent will output Chain-of-Thought that mentions informations that are essential for generating combinations and constraints that are essential for filtering plans.
2. Structured output - The agent will provide the combinations and constraints based on the few-shot examples, as well as their corresponding field description.

Here is the Chain-of-Thought (CoT) of Planning Agent:
<cot>

Here is the structured output of Planning Agent:
<structured_output>

Here is the planning instructions of Planning Agent:
<planning>

Your main job is as follows:
1. The structured output of Planning Agent might be missing some informations in "combinations" and "constraints". This might be due to misplaced of information at a wrong key.
2. You must go through each of the point in the CoT of planning agent and mention whether each point below "Informations that are essential for generating combinations" is missing in "combinations" and each point below "Constraints that are essential for filtering plans" is missing in "constraints" in point form. You write these in your CoT.
3. If the information is essential at both keys, the information must exist at both keys. Hence, you must duplicate the information so it exists at both keys. For example, the information exists in "constraints" but not "combinations", then you copy that corresponding key and values to "combinations". You should copy the entire key and values.
4. Finally, rewrite the structured output and planning instructions.
5. If any information related to initial state exists, both "combinations" and "constraints" must include those informations. This is to help both "combination" and "constraints" take these information into account when creating and filtering plans.

Your output format is as follows:
<start_of_COT>
<Mention what is missing in point form>
<end_of_COT>

<start_of_structured_output>
<Your structured output>
<end_of_structured_output>

<start_of_planning>
<your planning>
<end_of_planning>


\end{tcblisting}

\clearpage

\section{Problem Optimization for Travel Planner}

\needspace{6\baselineskip}

\begin{tcblisting}{title=Code to auto filter and prune reference data, listing only, breakable}
    def check_sufficient(self, filtered_reference_data, minimum_requirement_item, key):
        minimum_requirement_item_dict = minimum_requirement_item[key] # City/from_to : number

        if(key=="transport"):
            parameter = "from_to"
        else:
            parameter = "City"

        city_or_transport_count = {}
        for cat in minimum_requirement_item_dict:
            city_or_transport_count[cat] = 0

        for item in filtered_reference_data:
            city_or_transport_count[item[parameter]] += 1

        for cat in city_or_transport_count:
            if(city_or_transport_count[cat] < minimum_requirement_item_dict[cat]):
                return False
        
        return True


    def filter_item(self, structured_output_full, reference_data, set_cover_param):
        structured_output = structured_output_full["constraints"]

        key_to_filter = {"restaurants": ["Cuisines"], "accommodations": ["room type", "house_rules"], "transport": ["mode"]}

        filtered_reference_data = reference_data.copy()

        remaining_structured_output = {}

        minimum_requirement_item = structured_output_full["combinations"]

        if("other_constraints" in structured_output_full["constraints"]):
            remaining_structured_output["other_constraints"] = structured_output_full["constraints"]["other_constraints"]
        
        if("accommodations" in structured_output_full["constraints"]):
            remaining_structured_output["accommodations"] = {}
            if("maximum occupancy" in structured_output_full["constraints"]["accommodations"]):
                remaining_structured_output["accommodations"]["maximum occupancy"] = structured_output_full["constraints"]["accommodations"]["maximum occupancy"]

            if("minimum nights" in structured_output_full["constraints"]["accommodations"]):
                remaining_structured_output["accommodations"]["minimum nights"] = structured_output_full["constraints"]["accommodations"]["minimum nights"]
            

        for key in key_to_filter:
            if(key not in structured_output):
                filtered_reference_data[key] = reference_data[key]
                continue

            for constraint in key_to_filter[key]:
                # if filtered data is under requirement. disable filtering for the key.
                before_filtering = filtered_reference_data[key].copy()
                
                if(constraint not in structured_output[key]):
                    continue

                if(constraint=="Cuisines"):
                    # need to retain only
                    candidate_data = filtered_reference_data[key]
                    remaining_data = []
                    if(len(structured_output[key][constraint])>0):
                        for item in candidate_data:
                            result = any(x_item == y_item for x_item in structured_output[key][constraint] for y_item in item[constraint])

                            if(result):
                                remaining_data.append(item)
                        
                        filtered_reference_data[key] = remaining_data
                    else:
                        filtered_reference_data[key] = candidate_data
                else:
                    # need to retain and filter. we filter first, then retain.
                    retain_conditions = []
                    filter_conditions = []

                    for option in structured_output[key][constraint]:
                        if(option[:3].lower()=="not"):
                            raw_option = option[4:].strip()
                            filter_conditions.append(raw_option)
                        else:
                            raw_option = option.strip()
                            retain_conditions.append(raw_option)


                    if(constraint=="room type" or constraint=="mode"):
                        candidate_data = filtered_reference_data[key]

                        remaining_data = []

                        if(len(filter_conditions)>0):
                            for item in candidate_data:
                                if(item[constraint] not in filter_conditions):
                                    remaining_data.append(item)
                        else:
                            remaining_data = candidate_data  

                        
                        second_stage_remaining_data = []
                        if(len(retain_conditions)>0):
                            for item in remaining_data:
                                if(item[constraint] in retain_conditions):
                                    second_stage_remaining_data.append(item)
                        else:
                            second_stage_remaining_data = remaining_data
                        
                        filtered_reference_data[key] = second_stage_remaining_data

                    else:
                        candidate_data = filtered_reference_data[key]
                        remaining_data = []

                        if(len(filter_conditions)>0):
                            for item in candidate_data:
                                item_conditions = item[constraint]
                                overlap_exists = set(item_conditions) & set(filter_conditions)
                                if(len(overlap_exists)==0):
                                    remaining_data.append(item)
                        else:
                            remaining_data = candidate_data

                        second_stage_remaining_data = []
                        if(len(retain_conditions)>0):
                            for item in remaining_data:
                                item_conditions = item[constraint]
                                is_sublist = all(x in retain_conditions for x in item_conditions)
                                if(is_sublist):
                                    second_stage_remaining_data.append(item)
                        else:
                            second_stage_remaining_data = remaining_data
                        
                        filtered_reference_data[key] = second_stage_remaining_data

                if(self.check_sufficient(filtered_reference_data[key], minimum_requirement_item, key)==False):
                    print("Revoking filter", key, constraint)
                    filtered_reference_data[key] = before_filtering

        # attractions should have unique city
        existing_city = set()
        filtered_attractions = []

        for attraction in filtered_reference_data["attractions"]:
            if(attraction["City"] not in existing_city):
                filtered_attractions.append(attraction)
                existing_city.add(attraction["City"])

        filtered_reference_data["attractions"] = filtered_attractions

        # minimum nights <=2
        filtered_accommodations = []
        for accommodation in filtered_reference_data["accommodations"]:
            if(accommodation["minimum nights"] <= 2):
                filtered_accommodations.append(accommodation)

        if(self.check_sufficient(filtered_accommodations, minimum_requirement_item, "accommodations")==False):
            print("Revoking filter", "accommodations", "minimum nights")
        else:
            filtered_reference_data["accommodations"] = filtered_accommodations

        required_cuisines = set_cover_param

        chosen = {}

        restaurants = filtered_reference_data["restaurants"]

        with open("filtered_items.json", "w") as f:
            json.dump(filtered_reference_data, f, ensure_ascii=False, indent=4)

        # Step 1: pick cheapest restaurant per required cuisine

        if(len(required_cuisines)>0):
            for cuisine in required_cuisines:
                candidates = [r for r in restaurants if cuisine in r["Cuisines"]]
                if not candidates:
                    raise ValueError(f"No restaurant found serving {cuisine}")
                cheapest = min(candidates, key=lambda x: x["Average Cost Per Person"])
                chosen[cheapest["name"]] = cheapest
        else:
            candidates = restaurants
            cheapest = min(candidates, key=lambda x: x["Average Cost Per Person"])
            chosen[cheapest["name"]] = cheapest

         # Step 2: group chosen by city
        city_groups = {}
        for r in chosen.values():
            city_groups.setdefault(r["City"], []).append(r)

        # Step 3: pad each city to 3 restaurants
        all_cities = set(r["City"] for r in restaurants)
        for city in all_cities:
            selected = city_groups.get(city, [])
            if len(selected) < 3:
                remaining = sorted(
                    [r for r in restaurants if r["City"] == city and r not in selected],
                    key=lambda x: x["Average Cost Per Person"]
                )
                selected.extend(remaining[:3 - len(selected)])
            elif len(selected) > 3:
                selected = sorted(selected, key=lambda x: x["Average Cost Per Person"])[:3]
            city_groups[city] = selected

        # Step 4: flatten back to a pruned list
        pruned_list = []
        for city, rs in city_groups.items():
            pruned_list.extend(rs)

        filtered_reference_data["restaurants"] = pruned_list
        
        return filtered_reference_data, remaining_structured_output

\end{tcblisting}

\begin{tcblisting}{title=Code to auto package parameters, listing only, breakable}
        def group_items_by_parameter(self, items_list, group_param):
        """
        Generic grouping based on the group_parameter mapping.
        items_list: list of item dicts
        group_param: string, e.g., 'City' or 'from_to'
        """
        grouped = defaultdict(list)

        for item in items_list:
            key = item[group_param]
            grouped[key].append(item)
        return grouped


    def build_generic_combinations(self, structure, items_raw, group_parameter):
        """
        structure: dict {"key": {"location": "count"}}
        items_raw: dict {"key": [list_of_dict_items]}
        group_parameter: dict {"key": "grouping_field"}
        
        Returns a list of valid combinations with all metadata intact.
        """
        # Step 0: Group items dynamically
        items_dict = {}
        for key, items_list in items_raw.items():
            param = group_parameter.get(key, "City")  # default fallback
            items_dict[key] = self.group_items_by_parameter(items_list, param)
        

        # Step 1: Generate possible selections per key and location
        selections_per_key = {}
        for key, loc_dict in structure.items():
            selections_per_key[key] = {}
            for loc, count_str in loc_dict.items():
                count = int(count_str)
                available_items = items_dict[key].get(loc, [])
                if not available_items:
                    selections_per_key[key][loc] = []
                    continue
                
                # Select combinations
                if count == 1:
                    selections = [[item] for item in available_items]
                else:
                    selections = list(itertools.combinations(available_items, count))
                selections_per_key[key][loc] = selections

        # Step 2: Cross-product across locations within each key
        key_combos = {}
        for key, loc_dict in selections_per_key.items():
            loc_keys = list(loc_dict.keys())
            loc_values = [loc_dict[loc] for loc in loc_keys]
            if all(loc_values):
                combos = list(itertools.product(*loc_values))
                mapped_combos = []
                for combo in combos:
                    mapped_combo = {loc_keys[i]: list(combo[i]) for i in range(len(loc_keys))}
                    mapped_combos.append(mapped_combo)
                key_combos[key] = mapped_combos
            else:
                key_combos[key] = []
        
        # Step 3: Cross-product across all keys
        all_keys = list(key_combos.keys())
        all_values = [key_combos[key] for key in all_keys if key_combos[key]]
        if not all_values:
            return []
        
        final_combos = []
        for combo in itertools.product(*all_values):
            plan = {all_keys[i]: combo[i] for i in range(len(all_keys))}
            final_combos.append(plan)
        
        return final_combos


\end{tcblisting}
